Decentralized Dynamic Stable Matching

We study decentralized computing of the player-optimal stable matching under unannounced player arrivals and departures. Without a common clock, arrival/departure events information, or direct communication, players can only make individual proposals to arms and observe individual accept/reject outcomes. We measure mismatch cost --- the number of rounds in which the realized matching differs from that round's POSM, as the time horizon $T$ grows. For known preferences, we develop a deterministic polynomial-time self-calibrating protocol with mismatch cost $O(t_*+K^2\log T)$, greatly improving the existing upper-bound $O(T^{1-1/K}(\log T)^{2/K})$. $K$ is the number of arms and $t_*$ the last event time in the problem instance. Each player runs the protocol using their own local time and proposal-outcome history, without knowing~$t_*$ or $T$. More generally, configuring our protocol with a non-decreasing polynomial-time-computable function $g(t)=\Omega(t)$ yields mismatch cost $O(g(t_*) + K^2 N_g(T))$, where $N_g(T)$ counts iterations of $t\mapsto t+g(t)$ below $T$. $g(t)$ reflects the protocol's convergence speed. The relationship between $g(t)$ and~$N_g(T)$ reflects the tradeoff between convergence speed and asymptotic mismatch cost. We show that any randomized protocol with convergence speed $g(t)\geq 1$ has worst-case expected cost $\Omega(t_* + N_g(T))$. Thus, up to a $K^2$ factor, our protocol with $g(t)=t$ is optimal among protocols with convergence speed $O(t_*)$. For unknown preferences on both sides, each player and arm observe their own sampled utilities after being matched. We develop a decentralized learning protocol with expected mismatch cost $O(t_*+K^4\Delta_{\mathrm{min}}^{-2}\log T)$, where $\Delta_{\min}$ measures the preference gaps. A complementary static-setting lower-bound adapted from the literature shows that dependencies on $T$ and $\Delta_{\min}$ are tight.

==> appendices/learning-lower-bounds.tex <==
\subsection{Statistical lower bounds and recovery in the learning model}
\label{app:learning-lower}

The proof of \cref{cor:learning-static-lower} combines the accepted-edge information bound in Section~\ref{sec:learning-lower:information} with the arm-side construction in Section~\ref{sec:learning-lower:arm-side}. Section~\ref{sec:learning-lower:program} develops a general information bound for the POSM objective, and Section~\ref{sec:learning-lower:one-player} gives a complementary player-side construction. Section~\ref{sec:learning-lower:recovery} combines statistical cost with hidden-departure recovery under an additional window condition. The population-prefix bound in Section~\ref{sec:learning-lower:prefix} uses a separate instance family; Section~\ref{sec:learning-lower:interpretation} compares the resulting bounds and objectives.

For the statistical bounds, we use independent Bernoulli rewards at both endpoints of each accepted edge, a subclass of the conditional-mean model. The protocol and its arm-service rules are fixed before the means are chosen; rejection supplies neither a reward observation nor an exogenous ranking oracle. These bounds hold even for a central controller that can choose any feasible matching and observe every accepted reward, and can therefore simulate every local state and decision of SC-PC. Theorem~\ref{thm:learning} makes SC-PC uniformly efficient in the sense of \cref{cor:learning-static-lower}. The recovery argument in Section~\ref{sec:learning-lower:recovery} reinstates the local information restrictions, under which departures are not announced.

\subsubsection{Information from accepted edges}
\label{sec:learning-lower:information}

An alternative can change the POSM while preserving the reward laws on every original POSM edge. Distinguishing such an alternative requires observations from other edges. We first express the information in those observations.

\paragraph{Transcript divergence.}
Let $\theta$ and $\lambda$ denote two static mean instances with the same population and endpoint means $\mu_{i,x}$ and $\pi_{x,i}$, as in Section~\ref{sec:model}. Let $N_{i,x}(T)$ count acceptances of edge $(i,x)$ in the first $T$ rounds. Write $\mathbb P_\theta^T$ for the transcript law and $D_\theta(T)$ for the POSM-mismatch cost under $\theta$. Write $\operatorname{KL}$ for relative entropy and $\operatorname{kl}$ for its Bernoulli specialization, both defined using natural logarithms. On the full observation transcript, the chain rule gives
\begin{equation}
 \operatorname{KL}(\mathbb P_\theta^T,\mathbb P_\lambda^T)
 =\sum_{i,x}\mathbb E_\theta N_{i,x}(T)
 \left\{\operatorname{kl}(\mu_{i,x}^{\theta},\mu_{i,x}^{\lambda})
             +\operatorname{kl}(\pi_{x,i}^{\theta},\pi_{x,i}^{\lambda})\right\}.
\label{eq:learning-lower:kl-transcript}
\end{equation}
Conditional on the same observed history, the protocol uses the same action and state-update laws in both instances. Only the distributions of newly observed endpoint rewards can differ, so all divergence accumulates through these observations. Rejections and local state transitions contribute no additional term. Equation \eqref{eq:learning-lower:kl-transcript} specializes the adaptive change-of-measure identity to two observations per accepted edge; see also \cite[Lemma 1]{KCG16}.

\paragraph{One-edge alternatives.}
Suppose edge $e$ is absent from the original POSM and present in the alternative POSM, and the two instances differ only in one endpoint mean on that edge, which changes from $p$ to $q$. Then
\[
              N_e(T)\le D_\theta(T),\qquad
              T-N_e(T)\le D_\lambda(T)
\]
pathwise in their respective instances. For a uniformly efficient protocol and every $\alpha\in(0,1)$, the event $A_T=\{N_e(T)<T/2\}$ satisfies
\[
 \mathbb P_\theta(A_T)=1-o(T^{\alpha-1}),\qquad
 \mathbb P_\lambda(A_T)=o(T^{\alpha-1}).
\]
This follows directly from Markov's inequality and the definition of uniform efficiency. Binary data processing and the bound on binary entropy imply
\[
 \operatorname{KL}(\mathbb P_\theta^T,\mathbb P_\lambda^T)
 \ge \mathbb P_\theta(A_T)\ln\frac1{\mathbb P_\lambda(A_T)}-\ln2.
\]
Divide by $\ln T$, take the lower limit, and then let $\alpha\downarrow0$. Using \eqref{eq:learning-lower:kl-transcript}, we obtain
\begin{equation}
 \liminf_{T\to\infty}\frac{\mathbb E_\theta N_e(T)}{\ln T}
                 \ge\frac1{\operatorname{kl}(p,q)}.
\label{eq:learning-lower:one-edge}
\end{equation}
Under this one-edge perturbation, the argument requires only a change in POSM membership; uniqueness of the stable matching is unnecessary. It also remains valid when the unchanged means are revealed to the controller. The constructions in Sections~\ref{sec:learning-lower:arm-side} and \ref{sec:learning-lower:one-player} will use instances with unique stable matchings.

\subsubsection{An information bound for the player-optimal objective}
\label{sec:learning-lower:program}

We now collect the information constraints into a lower bound for the POSM objective. Fix the population and consider the full class of Bernoulli instances with strict preferences and means in $(0,1)$. Uniform efficiency is required throughout this class. For an edge $e=(i,x)$, write $\mu_e=\mu_{i,x}$ and $\pi_e=\pi_{x,i}$. Let $\mathcal M$ be the finite set of feasible partial matchings and define
\[
 k_e(\theta,\lambda)=\operatorname{kl}(\mu_e^\theta,\mu_e^\lambda)+\operatorname{kl}(\pi_e^\theta,\pi_e^\lambda),
 \qquad k_M(\theta,\lambda)=\sum_{e\in M}k_e(\theta,\lambda).
\]
If $m_\lambda^*\ne m_\theta^*$, consider the event that $m_\theta^*$ is played on more than $T/2$ rounds. Uniform efficiency gives probability $1-o(T^{\alpha-1})$ under $\theta$ and $o(T^{\alpha-1})$ under $\lambda$. Applying the preceding data-processing argument yields
\begin{equation}
 \liminf_{T\to\infty}
     \frac{\operatorname{KL}(\mathbb P_\theta^T,\mathbb P_\lambda^T)}{\ln T}\ge1.
\label{eq:learning-lower:posm-kl}
\end{equation}
We focus on alternatives that change the POSM while preserving every reward law observed under the original POSM:
\[
 \mathcal A_{\mathrm{POSM}}(\theta)=
 \{\lambda:m_\lambda^*\ne m_\theta^*,\quad
                   k_e(\theta,\lambda)=0\ \text{for every }e\in m_\theta^*\}.
\]

\begin{proposition}[A structured POSM information program]
\label{prop:learning-lower:program}
Every uniformly efficient protocol satisfies
\[
       \liminf_{T\to\infty}\frac{\mathbb E_\theta D(T)}{\ln T}
                    \ge c_{\mathrm{POSM}}(\theta),
\]
where
\begin{equation}\begin{aligned}
 c_{\mathrm{POSM}}(\theta)&=\inf_{w_M\ge0}\ \sum_{M\ne m_\theta^*}w_M,\\
 \text{subject to}\quad
 &\sum_{M\ne m_\theta^*}w_M k_M(\theta,\lambda)\ge1
       \qquad\text{for every }\lambda\in\mathcal A_{\mathrm{POSM}}(\theta).
\end{aligned}\label{eq:learning-lower:program}
\end{equation}
The value is zero if the alternative set is empty and $+\infty$ if the constraints are infeasible. The proposition does not assert that this lower bound is attainable.
\end{proposition}
\begin{proof}
Let $N_M(T)$ count the rounds whose accepted matching is $M$, and put $w_M(T)=\mathbb E_\theta N_M(T)/\ln T$ for $M\ne m_\theta^*$. The sum of these weights is $\mathbb E_\theta D(T)/\ln T$. For each alternative in the specified set, playing $m_\theta^*$ contributes no divergence. Equations \eqref{eq:learning-lower:kl-transcript} and \eqref{eq:learning-lower:posm-kl} therefore give
\[
       \liminf_T\sum_{M\ne m_\theta^*}w_M(T)k_M(\theta,\lambda)\ge1.
\]
If the normalized cost has infinite lower limit, the result is immediate. Otherwise, take a sequence along which it converges to its finite lower limit. Nonnegativity bounds every coordinate along this sequence. Since $\mathcal M$ is finite, a subsequence converges coordinatewise to a nonnegative vector $w$. For each fixed alternative, the corresponding finite linear form converges as well, so $w$ satisfies its constraint. This same limiting vector is feasible for every alternative, and its objective equals the chosen lower limit.
\end{proof}

\paragraph{Comparison with binary stability.}
Basu's binary-stability program fixes the means on the union of all originally stable edges and considers alternatives with no stable matching in common with the original instance \cite[Definition 5.1 and Theorem 5.2]{basu2025super}. When the Bernoulli parameter class and the matching permissions are the same, each such alternative belongs to $\mathcal A_{\mathrm{POSM}}(\theta)$. Every original stable matching gives zero information against it. Removing the stable-matching coordinates from a feasible POSM vector therefore produces a feasible binary-stability vector with no larger objective. Under these common conditions, $c_{\mathrm{POSM}}(\theta)\ge c_{\rm binary}(\theta)$. The next two results show why this comparison can be strict.

\begin{corollary}[Positive information cost at every strict interior instance]
\label{cor:learning-lower:positive}
For a nonempty fixed population and $K\ge2$, every strict interior instance in the full two-sided unknown-mean class has $c_{\mathrm{POSM}}(\theta)>0$.
\end{corollary}
\begin{proof}
Choose a player $i$ and an arm $x\ne m_\theta^*(i)$. Increase both endpoint means on $(i,x)$ above the other means at their respective endpoints, keeping both below one. The endpoints become mutual first choices, so their pair belongs to every stable matching. The POSM changes, while all reward laws on original POSM edges remain fixed. With $k=k_{ix}(\theta,\lambda)\in(0,\infty)$, the constraint from this alternative is
\[
                 k\sum_{M:(i,x)\in M}w_M\ge1.
\]
Thus every feasible vector has objective at least $1/k>0$.
\end{proof}

\paragraph{A strict separation.}
The following two-player, two-arm example separates the information bounds: every edge belongs to a stable matching, yet meeting the POSM objective requires further information. For $0<\delta\le1/8$, let
\[
\begin{array}{c|cc}
 &0&1\\\hline
 \mu_{1,\cdot}&1/2&1/2-\delta\\
 \mu_{2,\cdot}&1/4&3/4
\end{array}
\qquad
\begin{array}{c|cc}
 &1&2\\\hline
 \pi_{0,\cdot}&1/4&3/4\\
 \pi_{1,\cdot}&3/4&1/4
\end{array}.
\]
The matching along the diagonal of the player-mean matrix is player-optimal, while the reversed matching is also stable. Their union contains every edge, so fixing all stable-edge laws leaves the binary program with no alternative and value zero. Now change only $\mu_{1,1}$ to $1/2+\varepsilon$, with $0<\varepsilon<1/4$. The reversed matching becomes uniquely stable, and the reward laws on the diagonal edges remain unchanged. Equation \eqref{eq:learning-lower:one-edge}, followed by $\varepsilon\downarrow0$, gives
\[
 \liminf_{T\to\infty}\frac{\mathbb E_\theta N_{1,1}(T)}{\ln T}
 \ge\frac1{\operatorname{kl}(1/2-\delta,1/2)}\ge\frac1{4\delta^2}.
\]
Each such acceptance incurs a POSM mismatch. In the original instance $E_1^*=\{0\}$, $E_2^*=\{1\}$, and $\Delta_{\min}=\delta$. Thus the binary program can give a zero lower bound even when meeting the POSM objective has a positive information cost. A zero value of that program does not imply that zero regret is achievable.

\subsubsection{Arm-side learning with all player means revealed}
\label{sec:learning-lower:arm-side}

\paragraph{The instance.}
With the player means revealed, uniform efficiency is required over all strict Bernoulli arm-mean instances sharing those same player means. Fix $K$ and $\Delta$ as in \cref{cor:learning-static-lower}. Let the players be $p_0,\ldots,p_{K-1}$ and the arms $0,\ldots,K-1$. Each player other than $p_0$ will form a mutual first-choice pair with a distinct arm, leaving $p_0$ its last choice. Reversing one arm's preference between its owner and $p_0$ changes the POSM; learning those comparisons will account for the lower bound. Choose player means
\[
 \mu_{p_0,j}=\frac12+(K-1-j)\Delta,
 \qquad
 \mu_{p_r,j}=\begin{cases}
       3/4,&j=r-1,\\
       1/8+(j+1)/(8K),&j\ne r-1,
      \end{cases}\qquad 1\le r<K.
\]
On each arm $j<K-1$, set
\[
 \pi_{j,p_{j+1}}=\frac12,\qquad
 \pi_{j,p_0}=\frac12-\Delta,\qquad
 \pi_{j,p_r}=\frac18+\frac r{8K}\quad(r\notin\{0,j+1\}).
\]
On the last arm, set $\pi_{K-1,p_0}=3/4$ and $\pi_{K-1,p_r}=1/8+r/(8K)$ for $r\ge1$. All means are interior and all local rankings are strict. In each pair $(p_r,r-1)$, $r\ge1$, the endpoints are mutual first choices, so the pair occurs in every stable matching. The remaining player $p_0$ receives arm $K-1$, giving a unique stable matching.

\paragraph{The relevant gap.}
For this instance,
\[
 E_{p_0}^*=\mathcal K,\qquad E_{p_r}^*=\{r-1\}\quad(r\ge1).
\]
Among the means of player $p_0$, the smallest positive difference is $\Delta$. For each other player, the reward gap between its assigned first choice and any other arm is at least $1/2$. At each arm $j$ other than the last, the only distinct players whose relevant sets both contain that arm are $p_0$ and $p_{j+1}$; the difference between their means at this arm is $\Delta$. The last arm belongs only to the remaining player's relevant set. Consequently $\Delta_{\min}=\Delta$ exactly.

\paragraph{Alternatives and information cost.}
For each $j<K-1$, change only $\pi_{j,p_0}$ to $1/2+\varepsilon$, where $0<\varepsilon<1/8$. All player means remain fixed. The endpoints of the other $K-2$ owner pairs remain mutual first choices. In the remaining market, $p_0$ prefers $j$ to $K-1$ and $j$ prefers $p_0$ to its former owner, so $(p_0,j)$ belongs to every stable matching. The displaced owner receives $K-1$, again giving a unique stable matching. For $N_j=N_{p_0,j}$, \eqref{eq:learning-lower:one-edge} implies
\[
 \liminf_{T\to\infty}\frac{\mathbb E N_j(T)}{\ln T}
       \ge\frac1{\operatorname{kl}(1/2-\Delta,1/2+\varepsilon)}.
\]
Let $\varepsilon\downarrow0$. Each acceptance of one of these edges in the original instance incurs a mismatch. Since the same player cannot be accepted at two arms in one round, $\sum_{j<K-1}N_j(T)\le D(T)$. For $p\in[3/8,1/2]$, the second derivative of $p\mapsto\operatorname{kl}(p,1/2)$ is $1/[p(1-p)]\le64/15$. Its value and first derivative vanish at $p=1/2$, so Taylor's theorem and $\Delta\le1/8$ give
\[
 \operatorname{kl}(1/2-\Delta,1/2)
 \le\frac{32}{15}\Delta^2
 <4(\ln2)\Delta^2.
\]
Converting the normalization in \eqref{eq:learning-lower:one-edge} to base two and summing therefore gives
\[
 \liminf_{T\to\infty}\frac{\mathbb E D(T)}{\log T}
 \ge\frac{(\ln2)(K-1)}{\operatorname{kl}(1/2-\Delta,1/2)}
 \ge\frac{K-1}{4\Delta^2}.
\]
All alternatives change only arm means. The construction therefore proves \cref{cor:learning-static-lower} even when all player means are revealed and accepted observations are centralized: the uncertainty responsible for the bound lies entirely on the arm side.

\subsubsection{A complementary one-player construction}
\label{sec:learning-lower:one-player}

A complementary player-side construction permits a gap range independent of the number of arms. For any $K\ge2$ and $0<\delta\le1/8$, take one permanent player $i$ with
\[
 \mu_{i,0}=\frac12,\qquad
 \mu_{i,x}=\frac12-\delta\left(1+\frac{x-1}{K-1}\right),\quad 1\le x<K.
\]
Every arm's mean for the sole player may be $\pi_{x,i}=1/2$. The unique POSM assigns the player to arm $0$; thus $E_i^*=\{0\}$ and $\Delta_{\min}=\delta$. Changing one $\mu_{i,x}$ to $1/2+\varepsilon$ and using \eqref{eq:learning-lower:one-edge} yields
\[
 \liminf_{T\to\infty}\frac{\mathbb E D(T)}{\ln T}
 \ge\sum_{x=1}^{K-1}\frac1{\operatorname{kl}(\mu_{i,x},1/2)}
 \ge\frac{K-1}{16\delta^2}.
\]
The last inequality follows because each deficit $1/2-\mu_{i,x}$ is smaller than $2\delta$.

This family allows a gap interval independent of $K$, while the preceding family isolates arm-side learning. Both comparisons fix the instance before taking the horizon limit; they are not uniform in jointly varying $T,K,\delta$. At every finite horizon, the deterministic bound $D(T)\le T$ still applies.

\subsubsection{Recovery and learning on the same fixed instance}
\label{sec:learning-lower:recovery}

The arm-side family also links learning to recovery. We now impose the model's local information restrictions: arms may retain local state and accepted statistics, but departures are not publicly announced. We adapt the hidden-departure argument from Section~\ref{sec:tradeoff-lower-proof} by coupling the executions until the first static mismatched round after a prescribed departure. Both the statistical argument and the recovery argument will bound the cost on this same static instance. Recall from \eqref{eq:budget-iteration-count} that $N_g(T)=\#\{j:r_j<T\}$, where $r_0=2$ and $r_{j+1}=r_j+g(r_j)$.

\begin{proposition}[A joint obstruction on the arm-side family]
\label{prop:learning-lower:joint}
Let $I_{K,\Delta}$ be the static instance of Section~\ref{sec:learning-lower:arm-side} and let $I_\tau$ delete $p_1$ at the predetermined round $\tau\ge2$. Define the expected post-deletion cost
\[
 L_\Pi(\tau,h)=\mathbb E\left[D_\Pi(\tau+h;I_\tau)-D_\Pi(\tau;I_\tau)\right].
\]
Let $g:\mathbb N_{\ge1}\to\mathbb N_{\ge1}$ be nondecreasing. Suppose the same local protocol is uniformly efficient and satisfies
\[
 L_\Pi(\tau,h)\le Ag(\tau)+C+\eta h\qquad(\tau\ge2,\ h\ge1)
\]
for fixed finite $A,C\ge0$ and $\eta\in(0,1)$. The constants $A$ and $C$ may depend on this fixed family, but not on $\tau$ or $h$. Then, with this instance fixed,
\begin{equation}
 \mathbb E D_\Pi(T;I_{K,\Delta})
 =\Omega_{A,C,\eta}\!\left(N_g(T)+(K-1)\Delta^{-2}\log T\right).
\label{eq:learning-lower:joint}
\end{equation}
The recovery requirement is a separate assumption on the fixed-mean deletion family.
\end{proposition}
\begin{proof}
\emph{Coupling after deletion.} Deleting $p_1$ preserves all other owner pairs and moves $p_0$ to the vacated arm $0$, changing the survivors' POSM. Couple the static and deletion executions using common algorithmic randomness and common rewards on accepted survivor edges. Until the first static mismatched round at or after deletion, each surviving player and its originally assigned arm have identical local states and observations in the two executions. No survivor visits the deleted player's original arm during this coupled prefix, so that arm's changed state cannot convey the deletion elsewhere. The unchanged survivor assignment differs from the new POSM, and every round of the coupled prefix is therefore mismatched in the deletion execution.

\emph{Packing disjoint windows.} Let $d$ be the expected static cost in the augmented interval $\{\tau,\ldots,\tau+h\}$. The probability of any static mismatch there is at most $d$. If none occurs, all $h$ recovery rounds $\tau+1,\ldots,\tau+h$ are mismatched in the deletion execution. Its expected recovery cost is therefore at least $h\max\{0,1-d\}$. The augmented interval includes the deletion round to allow for detection in that round. The recovery condition therefore bounds the static expected cost below by a positive constant whenever $h$ is at least $2(Ag(\tau)+C)/(1-\eta)$. Using $g\ge1$ to absorb $C$ into the coefficient $A+C$, put
\[
          q=\max\{1,\lceil2(A+C)/(1-\eta)\rceil\}.
\]
Set $x_0=2$ and $x_{j+1}=x_j+qg(x_j)+1$. Apply the recovery bound at $\tau_j=x_j$ with $h_j=qg(x_j)$ and charge the disjoint augmented intervals $[x_j,x_{j+1})$. Monotonicity and $g\ge1$ give $x_j\le r_{(q+1)j}$, so the endpoint count in Section~\ref{sec:tradeoff-lower-proof} gives
\[
 \mathbb E D_\Pi(T;I_{K,\Delta})
 \ge\frac{1-\eta}{2}\,\max\{0,N_g(T)/(q+1)-1\}.
\]
\Cref{cor:learning-static-lower} also bounds this same expectation below by $(K-1)\Delta^{-2}\log T/8$ for all sufficiently large $T$. The maximum of two nonnegative quantities is at least half their sum, and $N_g(T)\to\infty$ absorbs the fixed subtraction. This proves \eqref{eq:learning-lower:joint}; the maximum inequality allows the rounds charged by the two arguments to overlap.
\end{proof}

For $g(t)=\Omega(t)$, $N_g(T)=O_g(\log T)$ by Section~\ref{sec:tradeoff-growth-proof}, so for fixed $K,\Delta,g$ the statistical term determines the horizon dependence of \eqref{eq:learning-lower:joint}. More generally, uniform efficiency imposes the following necessary condition on the recovery allowance.

\begin{proposition}[Necessary growth of the recovery allowance]
\label{prop:learning-lower:allowance}
Suppose a local uniformly efficient protocol satisfies the preceding recovery condition on one fixed static/deletion family for which the survivors' POSM changes. Then $N_g(T)=o(T^\alpha)$ for every $\alpha>0$. For a finite nondecreasing integer function $g\ge1$, this count condition is equivalent to
\begin{equation}
                   \liminf_{t\to\infty}\frac{\log g(t)}{\log t}\ge1.
\label{eq:learning-lower:allowance}
\end{equation}
\end{proposition}
\begin{proof}
The packing bound applies to every such fixed family, and uniform efficiency gives the necessary count condition. To establish its equivalence with \eqref{eq:learning-lower:allowance}, put $n=N_g(T)$, with the orbit $r_0=2$, $r_{j+1}=r_j+g(r_j)$. Then $r_n\ge T$ and $r_j<T$ for $j<n$, so
\[
                  T-2\le r_n-2=\sum_{j<n}g(r_j)\le n g(T).
\]
If the count condition holds, then $n\le T^\varepsilon$ eventually for each $\varepsilon>0$, which proves \eqref{eq:learning-lower:allowance}.

Conversely, \eqref{eq:learning-lower:allowance} implies $g(x)\ge x^{1-\varepsilon}$ eventually for each $0<\varepsilon<1$. In a dyadic interval $[2^j,2^{j+1})$, consecutive orbit points are separated by at least $2^{j(1-\varepsilon)}$, so the interval contains at most $1+2^{j\varepsilon}$ points. Summing these bounds gives $N_g(T)=O_\varepsilon(T^\varepsilon)$. For any prescribed $\alpha>0$, choose $\varepsilon<\alpha$.
\end{proof}

Thus a polynomially sublinear allowance \(g(t)=O(t^{1-\varepsilon})\) is incompatible with uniform efficiency under the stated recovery condition on the same fixed family. Uniform efficiency is stronger than vanishing average cost, so the known-preference question in \cref{sec:lower-bounds} remains separate.

Some allowances just below linear growth do satisfy the necessary condition: for example, \(g(t)=\lceil t/\ln(t+2)\rceil\) for \(t\ge1\), satisfies \eqref{eq:learning-lower:allowance} and has \(N_g(T)\sim\tfrac12(\ln T)^2\). Indeed, writing \(y_j=\ln r_j\) gives \(y_{j+1}-y_j\sim1/y_j\), and hence \(y_{j+1}^2-y_j^2\to2\); the stated count follows by summation. A matching learning upper bound would require a further construction.

\subsubsection{The separate cost of the population prefix}
\label{sec:learning-lower:prefix}

To account for the population prefix, consider the following arrival sequence. For an integer $t_*\ge1$, let a new player arrive in every round $1,\ldots,t_*$, replacing its predecessor; the last one remains forever. In this separate construction, each entrant's player means are unknown when its first proposal is chosen. Choose each new player's best arm independently and uniformly in advance by permuting a fixed strictly ordered set of interior Bernoulli means. Before that player's first proposal, no sample from its reward distributions is available. Set, for example,
\[
         \pi_{x,p_r}=\frac14+\frac{r}{2(t_*+1)},\qquad r=1,\ldots,t_*,
\]
at every arm. These means give each arm a strict ranking of players and reveal nothing about the new player's independently chosen permutation.

Even a central controller with all earlier observations chooses the new player's best arm with probability at most $1/K$. With only one player present, that arm is the POSM assignment. Average over the preselected means, then fix a selection whose expected cost is at least this average. This gives a legal oblivious instance with last event at $t_*$ and
\[
                           \mathbb E D(t_*)\ge(1-1/K)t_*.
\]
The case $t_*=1$ is a static instance initialized in round $1$. This construction gives a lower bound on the cost accumulated during the population prefix, on a separate instance family. It does not bound the rate of recovery after an event. Adding this cost to the static statistical lower bound would require a joint construction.

\subsubsection{Interpretation of the comparison}
\label{sec:learning-lower:interpretation}

On the hard family in Section~\ref{sec:learning-lower:arm-side}, the stable matching is unique, so unstable-round loss and POSM-mismatch loss coincide. The information program in Section~\ref{sec:learning-lower:program} extends the comparison to markets with several stable matchings: it charges a stable assignment whenever that assignment is not player-optimal. This distinction accounts for the separation from the binary-stability lower bound of \cite{basu2025super}.

Reward-regret results, such as those for common arm priorities in \cite{SBA21}, measure loss through reward differences, whereas $D(T)$ charges the whole mismatched market once per round. The gap dependence for one loss cannot be transferred directly to the other. For POSM mismatch, the upper bound and the displayed lower-bound families agree in their logarithmic horizon and inverse-square gap orders for fixed $K$. The optimal dependence on the number of arms remains open.


==> appendices/tradeoffs/accounting.tex <==
% \subsection{All-prefix accounting and the main theorem}
% \label{sec:proof-accounting}

% We establish \cref{thm:known} through the following quantitative bound. With the constants in \eqref{eq:parameters} and \eqref{eq:maintenance-window-budget}, for every integer \(K\ge2\), every legal finite-event instance \(I\), and every integer horizon \(T\ge0\), the same protocol satisfies
% \begin{equation}
%   D(T;I)\le
%   \min\!\left\{T,\,
%   32(u+H)+U\left[1+\left\lceil\log_2(T+2)\right\rceil\right]\right\},
%   \qquad T\ge0.
%   \label{eq:all-prefix-bound}
% \end{equation}

% \begin{proof}[Proof of \cref{thm:known}]
% Fix \(I,T\). If the final market is nonempty, \eqref{eq:recovery-time} gives a calibrated handoff at \(V_2\le32(u+H)\). Charge every earlier round at one. Starting with the second mature output at \(m=0\), \cref{lem:maintenance} gives \(L_m\ge2^mH\). A maintenance window beginning at \(Q_m=o_m+L_m<T\) thus has \(2^mH\le Q_m<T\), so at most
% \begin{equation}
%   1+\left\lceil\log_2(T+2)\right\rceil
%   \label{eq:maintenance-window-count}
% \end{equation}
% windows have begun. Each costs at most \(U\), including an unfinished final window. Adding these charges proves \eqref{eq:all-prefix-bound} for \(T\ge V_2\), using also \(D(T;I)\le T\).

% For \(T<V_2\), use \(D(T;I)\le T<V_2\le32(u+H)\). This covers prefixes before the last event: \(u=t_*+1\) still refers to the full instance path. If the final market is empty, no cost occurs after its last event, so \(D(T;I)\le\min\{T,u\}\). Thus \eqref{eq:all-prefix-bound} holds for every \(T\ge0\), including \(T=0\).

% For \(K\ge2\), \(U=2K^2+14K\le9K^2\), and
% \begin{equation}
%   32H+2U=512K^2+72-(K-2)(380K+92)\le512K^2+72.
%   \label{eq:constants-all-prefix}
% \end{equation}
% Using \(1+\lceil\log_2(T+2)\rceil\le2+\ln(T+2)/\ln2\), \(u\ge1\), and \(9/\ln2<13\),
% \[
% \begin{aligned}
%   D(T;I)&\le32u+512K^2+72+\frac9{\ln2}K^2\ln(T+2)\\
%         &\le512(u+K^2)+13K^2\ln(T+2).
% \end{aligned}
% \]
% Since \(\ln(T+2)\ge\ln2\), this is \(O(u+K^2\log(T+2))\) with absolute constants. The protocol and constants are independent of \(I,T\).
% \end{proof}

% For fixed \(K\) and a fixed legal finite-event instance \(I\), \(u<\infty\) is constant, so the all-prefix bound gives \(D(T;I)/T\to0\), even with indefinitely continuing maintenance.


==> appendices/tradeoffs/general-budgets.tex <==
\subsection{Compiling a general recovery scale}
\label{sec:tradeoff-upper-proof}

We construct the replay-length rule in \cref{lem:known-scale-rule}, prove its recovery and iteration bounds, and then record finite-horizon estimates and the post-event recovery guarantee.

\paragraph{Construction of the waiting rule.}
Fix a nondecreasing, polynomial-time computable function \(g:\mathbb N_{\ge1}\to\mathbb N_{\ge1}\) with \(g(t)=\Omega(t)\), and put
\[
 M_g=\max\left\{1,\sup_{t\ge1}\frac{t}{g(t)}\right\}<\infty.
\]
The asymptotic linear lower bound controls the ratios for all sufficiently large \(t\), and positivity controls the remaining finite set. The constant \(M_g\) is used only in the analysis. Define \(F_g:\mathbb N_{\ge1}\to\mathbb N_{\ge1}\) by
\begin{align}
 s_0&=H, &s_{j+1}&=s_j+g(s_j),\nonumber\\
 A_g(x)&=\max\bigl(\{g(s_j)-s_j:64s_j\le x\}\cup\{0\}\bigr),
 &F_g(x)&=H+2x+A_g(x).
 \label{eq:budget-waiting-rule}
\end{align}
The maximum is nonnegative and nondecreasing in \(x\), even though the individual differences need not increase with \(j\). Hence \(F_g\) is nondecreasing and satisfies \eqref{eq:general-wait-condition}.

Since \(s_{j+1}\ge(1+1/M_g)s_j\), evaluation visits \(O_g(1+\log(x+1))\) eligible scales. It calls \(g(s_j)\) only while \(64s_j\le x\), and maintains the maximum of the differences. The assumed polynomial-time computability of \(g\), together with integer additions and comparisons, therefore gives a polynomial-time evaluation of \(F_g\). The protocol \(\Pi_g\) uses \eqref{eq:general-wait-update} with this function, fixed by \(K,g\) before the instance and horizon; it does not need \(M_g\) as an input.

\begin{proof}[Proof of \cref{lem:known-scale-rule}]
The construction above is polynomial-time computable and satisfies the waiting-rule condition. We bound the recovery prefix and then compare the iterates of this rule with those of the given scale.

\paragraph{Bounding the recovery prefix.}
The recovery map is
\[
 \Psi_{F_g}(x)=3x+6H+A_g(x+H).
\]
We show
\begin{equation}
 \Psi_{F_g}^{\circ3}(t+1)\le C_g(t),\qquad
 C_g(t)=
 \begin{cases}
  105H,&1\le t<H,\\
  118(t+g(t)),&t\ge H.
 \end{cases}
 \label{eq:budget-recovery-envelope}
\end{equation}
For an integer \(t\ge H\), choose \(s_j\le t<s_{j+1}\) and put \(a=s_{j+1}\). Then
\[
 t+1\le a=s_j+g(s_j)\le t+g(t),\qquad H\le a.
\]
Whenever \(z+H<64a\), only indices \(k\le j\) can be activated, so \(A_g(z+H)\le\max_{k\le j}s_{k+1}=a\). Writing \(z_0=t+1\) and \(z_{i+1}=\Psi_{F_g}(z_i)\) gives
\[
 \begin{array}{lll}
 z_0+H\le2a,&z_1\le10a,\\
 z_1+H\le11a,&z_2\le37a,\\
 z_2+H\le38a,&z_3\le118a\le118(t+g(t)).
 \end{array}
\]
Every input stays below \(64a\). For \(1\le t<H\), \(z_0\le H\), and the three inputs to \(A_g\) are at most \(2H,10H,34H\), below the first threshold \(64H\). Thus all three additional terms vanish and
\[
 z_3=27(t+1)+78H\le105H.
\]
This proves \eqref{eq:budget-recovery-envelope} without any bound on \(g(t+1)/g(t)\). The function \(C_g\) is nondecreasing, including at \(H\).

\paragraph{Counting maintenance windows.}
Let \(b_0=H\) and \(b_{j+1}=F_g(b_j)\). Since \(F_g(x)\ge2x\), six iterations from \(s_j\) reach at least \(64s_j\), and
\[
 F_g(64s_j)\ge H+128s_j+g(s_j)-s_j
             \ge s_j+g(s_j)=s_{j+1}.
\]
Monotonicity therefore gives
\[
 b_{7j}\ge s_j,\qquad
 N_{F_g}(T)\le7\#\{j:s_j<T\}\le7N_g(T).
\]
Indeed, if \(m=\#\{j:s_j<T\}\), then \(b_{7m}\ge s_m\ge T\); also \(r_0=2\le H=s_0\) and monotonicity imply \(r_j\le s_j\). These comparisons include horizons equal to an iterate.

Since \(t\le M_g g(t)\) and \(H\le16K^2\), \eqref{eq:budget-recovery-envelope} gives the first bound in \cref{lem:known-scale-rule}, with a constant depending only on \(g\). The identity \(b_j=F_g^{\circ j}(H)\) gives the second with the universal constant \(7\). When \(g(t)=t\), every difference in \(A_g\) vanishes, so \(F_g(x)=H+2x\) for all \(x\ge1\).
\end{proof}

\paragraph{Finite-horizon estimates.}
Combining the two bounds above with \cref{lem:general-wait-interface} gives
\begin{equation}
 D_{\Pi_g}(T;I)
 \le\min\{T,118(t_*+g(t_*))+105H+7U N_g(T)\}.
 \label{eq:budget-finite-dynamic}
\end{equation}
For a static instance, \(t_*=1<H\), so the stronger bound is
\begin{equation}
 \sup_{I:\,t_*=1}D_{\Pi_g}(T;I)\le105H+7U N_g(T).
 \label{eq:budget-finite-static}
\end{equation}
Since \(H\le16K^2\), \(U\le9K^2\), and \(t_*\le M_g g(t_*)\), the dynamic estimate is \(O_g(g(t_*)+K^2[1+N_g(T)])\), with a constant independent of \(K,I,T\). The static estimate has constants uniform in \(K,g,I,T\). All shorter prefixes, including \(T=0\), and the empty-market case are covered by the interface. The proof of \cref{thm:general-budget-upper} in \cref{sec:known-analysis} absorbs the startup term and handles the small horizons.

\begin{proof}[Proof of \cref{cor:flexible-sublinear}]
We first bound the cost after calibration, then include the recovery prefix and choose the accuracy coefficients.

\paragraph{Cost after calibration.}
We verify the window guarantee used in \cref{sec:tradeoff-problem} directly from the actual maintenance windows. Fix \(\eta\in(0,1)\). The interface recurrences give
\[
 L_j\ge(2^{j+1}-1)H,\qquad
 Q_{j+1}-Q_j=c_j+L_{j+1}\ge(2^{j+2}-1)H.
\]
Every \([Q_j,V_{j+1})\) costs at most \(U\), and \(Q_0>V_{\mathrm{cal}}\). Put
\[
 m_\eta=\min\{m\in\mathbb Z_{\ge0}:(2^{m+2}-1)H\ge U/\eta\},\qquad
 Q_{K,\eta}=(m_\eta+1)U.
\]
Charge the first \(m_\eta\) windows separately. Later starts are at least \(U/\eta\) apart, so at most \(1+\eta h/U\) occur in any \(h\) consecutive rounds. In particular,
\begin{equation}
 D_{\Pi_g}(V_{\mathrm{cal}}+h;I)-D_{\Pi_g}(V_{\mathrm{cal}};I)
 \le Q_{K,\eta}+\eta h \qquad(h\ge0).
 \label{eq:budget-tail-discount}
\end{equation}
This difference counts rounds \(V_{\mathrm{cal}}+1,\ldots,V_{\mathrm{cal}}+h\). Because \(U/H\le1\), \(Q_{K,\eta}=O(K^2[1+\log(1/\eta)])\), independently of \(g\).

\paragraph{The post-event recovery window.}
Let \(\tau=t_*\) and \(a=V_{\mathrm{cal}}-\tau\) in a nonempty final market. The first \(a\) rounds of the event-excluding window cost at most \(a\le C_g(\tau)\). Splitting a longer window at \(V_{\mathrm{cal}}\) and using \eqref{eq:budget-tail-discount} gives, for every \(h\ge1\),
\begin{equation}
 L_{\Pi_g}(h;I)
 \le \min\{h,C_g(t_*)+Q_{K,\eta}+\eta h\}.
 \label{eq:budget-finite-recovery}
\end{equation}
Empty final markets have zero post-event cost.

\paragraph{Recovery coefficients.}
For \(0<\varepsilon<1\), take \(\eta=\varepsilon/2\) and
\[
 c_\varepsilon=
 \frac{2(118(1+M_g)+105H+Q_{K,\varepsilon/2})}{\varepsilon}>0.
\]
Since \(g(t_*)\ge1\) and \(C_g(t_*)\le118(1+M_g)g(t_*)+105H\), the condition \(h\ge c_\varepsilon g(t_*)\) implies \(L_{\Pi_g}(h;I)\le\varepsilon h\). For \(\varepsilon\ge1\), the claim follows from \(L_{\Pi_g}(h;I)\le h\). Thus the same \(\Pi_g\) has sublinear mismatch cost relative to \(g\); its rule has no accuracy parameter. In particular, the positive coefficient
\begin{equation}
 c^{\star}_{K,g}=4(118(1+M_g)+105H+Q_{K,1/4})=O_g(K^2)
 \label{eq:common-half-recovery}
\end{equation}
is valid uniformly over instances for each fixed \(K,g\). This is the threshold used for the common-coefficient class in \cref{cor:uniform-minimax-maintenance}.
\end{proof}

\paragraph{Comparison of integer scales.}
The growth examples in the next section use integer representatives of the displayed real-valued shapes. The following comparison shows that representatives within constant factors have the same iteration-count order. For nondecreasing positive integer scales \(g\le\widetilde g\le c g\) with \(g(t)=\Omega(t)\), put
\[
 Q_g(x)=x+g(x),\qquad
 d=\max\{1,\lceil c\rceil\}.
\]
Monotonicity gives \(Q_g^{\circ d}(x)\ge x+d g(x)\ge x+\widetilde g(x)\), and hence
\[
 Q_g(x)\le Q_{\widetilde g}(x)\le Q_g^{\circ d}(x).
\]
Iterating from \(2\) gives \(N_{\widetilde g}(T)\le N_g(T)\le dN_{\widetilde g}(T)\). For two nondecreasing positive integer scales with at least linear asymptotic growth and within constant factors, apply this comparison to their pointwise minimum and maximum. Thus their iteration counts have the same order even when neither scale dominates the other everywhere. The comparison is a growth statement; computational admissibility is the separate hypothesis in \cref{thm:general-budget-upper}, verified for the integer representatives in \cref{sec:tradeoff-growth-proof}.


==> appendices/tradeoffs/known-preferences.tex <==
% !TeX root = ../main.tex
\section{Details for Tracking with Known Preferences}
\label{app:known-proofs}
\label{sec:proof}
This appendix gives the local state definitions and the coordination arguments underlying \cref{lem:known-recovery,lem:known-maintenance}. Their proofs appear in \cref{sec:proof-recovery,sec:proof-maintenance}; \cref{sec:tradeoff-upper-proof} proves the replay-rule construction in \cref{lem:known-scale-rule}. The resulting proofs of \cref{thm:general-budget-upper,thm:known} are in \cref{sec:known-analysis}.

For the analysis, permit any nondecreasing computable waiting rule \(F:\mathbb N_{\ge1}\to\mathbb N_{\ge1}\) satisfying
\begin{equation}
 F(x)\ge H+2x.
 \label{eq:general-wait-condition}
\end{equation}
Keep every control rule of Algorithm~\ref{alg:scda-core}, replacing only the output update by
\begin{equation}
 y\leftarrow\text{the arm just proposed to},\qquad
 L\leftarrow F(a-\ell),\quad q\leftarrow a+L,\quad \ell\leftarrow a.
 \label{eq:general-wait-update}
\end{equation}
Every actual output uses the old \(\ell\), including an incorrect output or a rejected final proposal. Initialization and the order of all round-start and feedback updates are unchanged. The original algorithm uses \(F(x)=H+2x\). The lemmas below apply to the general rule.

\input{appendices/tradeoffs/local-protocol}
\input{appendices/tradeoffs/mature-executions}
\input{appendices/tradeoffs/sweep-isolation}
\input{appendices/tradeoffs/recovery}
\input{appendices/tradeoffs/maintenance}
\input{appendices/tradeoffs/accounting}


==> appendices/tradeoffs/local-protocol.tex <==
\subsection{Local state, auxiliary operations, and round order}
\label{sec:local}

We give the state definitions, equivalent auxiliary operations, and round order used to analyze \cref{alg:scda-core}, including histories that do not satisfy the mature-entry conditions. In \cref{eq:sweep}, \(\sigma_{2j-1}=0,\ \sigma_{2j}=j\) for \(1\le j\le K-1\), and the last two entries are zero.

The persistent state of player \(i\) consists of its ranking and \(a,y,\ell,\rho\). Here \(\rho\) is the length of the current consecutive suffix of actual accepted BUS proposals, capped at \(J\), and is updated in every mode. At birth,
\begin{equation}
  a=\ell=\rho=0,\qquad y=p_i(1),\qquad m=\SEEK .
  \label{eq:initialization}
\end{equation}
The temporary state consists of the mode \(m\), a scheduled next-round mode \(\nu\), a flag \(\mathit{seenR}\) recording whether this visit to \(\SEEK\) has seen a BUS rejection, a scan position \(s\) and block-success flag \(\mathit{blockOK}\), work counters \(h,k\), and the replay deadline \(q\). At a work action, \(h=0,\ldots,J-1\) counts completed rounds of that invocation, so the current action is work round \(h+1\).

\paragraph{Mode entry.}
The operation \(\operatorname{Enter}(m')\) first saves the requested mode \(m'\), then sets \(m\gets m'\) and \(\nu\gets\none\), clears the old mode-specific state, and leaves \(a,y,\ell,\rho\) unchanged. Thus a call \(\operatorname{Enter}(\nu)\) uses the pending mode before clearing it. It initializes the new mode as follows:
\[
\begin{array}{c|l}
  m' & \text{new mode-specific state}\\ \hline
  \SEEK   & \mathit{seenR}\gets\false\\
  \SWEEP  & s\gets 1,\quad \mathit{blockOK}\gets\true\\
  \WORK   & h\gets 0,\quad k\gets 1\\
  \REPLAY & \text{retain the deadline }q\text{ just computed at output}.
\end{array}
\]
Only a real work output updates \(\ell\). In particular, returning to \(\SEEK\) discards the old rejection flag but preserves the continuous BUS counter \(\rho\). Entering \(\REPLAY\) discards the other temporary state while retaining \(q\).

\paragraph{Proposal and feedback.}
The operation \(\operatorname{Pull}(x)\) makes one real proposal to arm \(x\), observes \(z\in\{\A,\R\}\) and the utility if accepted, updates
\[
  \rho\gets
  \begin{cases}
    \min\{J,\rho+1\},&x=\BUS\text{ and }z=\A,\\
    0,&\text{otherwise},
  \end{cases}
\]
and returns \(z\). This update applies in every mode and precedes the mode-specific feedback rules, so the AA handoff uses the updated value of \(\rho\).

\paragraph{Sweep advancement.}
The operation \(\operatorname{AdvanceSweep}(z)\) is called only in \(\SWEEP\) after a BUS rejection has been ruled out. It first sets \(\mathit{blockOK}\gets\mathit{blockOK}\wedge(z=\A)\), then applies exactly one of the following updates:
\begin{enumerate}[label=(\roman*)]
  \item If \(s<2K\), set \(s\gets s+1\).
  \item If \(s=2K\) and \(\mathit{blockOK}=\true\), set \(\nu\gets\WORK\).
  \item If \(s=2K\) and \(\mathit{blockOK}=\false\), set \(s\gets1\) and \(\mathit{blockOK}\gets\true\).
\end{enumerate}
A non-BUS rejection therefore marks the block as failed without rewinding its position. A failed block restarts at its first action in the next round. On a BUS rejection, the main controller instead sets \(\nu\gets\SEEK\) and skips this operation, including at \(s=2K\); this branch takes priority over the block-completion test.

\paragraph{Work action.}
The local action-selection function is
\[
  \operatorname{WorkArm}_i(h,k)=
  \begin{cases}
    \PARK,&0\le h<2K,\\
    p_i(1),&2K\le h\le4K,\\
    p_i(k),&4K<h<J.
  \end{cases}
\]
These are the \phase{Park}, \phase{Top}, and \phase{DA} portions of \(\WORK\). The main controller advances \(k\) only after a rejection in a nonfinal \phase{DA} round. In the final round it saves the actual proposed arm regardless of feedback and computes \(L\) using the old \(\ell\) before assigning \(\ell\gets a\), exactly as in \cref{eq:output}.

At every actual output, \(a-\ell\ge1\): the first output has \(\ell=0\) and \(a\ge J-1>0\), and subsequent outputs occur in strictly later local rounds than the output recorded in \(\ell\).

\paragraph{Round order.}
At each round's start, the environment applies entries and exits. This is not an event notification available to the player. Each present player then executes its previously scheduled mode change, checks replay expiration, and checks scan qualification, in that order. Scan qualification is checked only in \(\SEEK\), so it neither interrupts \(\WORK\) nor extends \(\REPLAY\). The player makes exactly one proposal, updates \(\rho\), handles feedback in the current mode, and increments \(a\).

Each loop iteration contains exactly one call to \(\operatorname{Pull}\). The operations \(\operatorname{Enter}\), \(\operatorname{AdvanceSweep}\), and \(\operatorname{WorkArm}_i\) are local state operations and consume no additional rounds.

Feedback-triggered mode changes take effect in the next round. Expiration and qualification checks affect the current round's action. A scheduled \(\WORK\) is therefore a pending transition, not an extra phase with its own actions. It arises only from a qualified AA pair in \(\SEEK\) or a successful complete scan.


==> appendices/tradeoffs/maintenance.tex <==
\subsection{Calibration and bounded maintenance}
\label{sec:proof-maintenance}

\paragraph{Calibration from actual consecutive outputs.}
Consider two mature executions in a fixed market of \(1\le n\le K\) players, consecutive in every player's actual output sequence. Label players by decreasing BUS preference, write \(m^*\) for the POSM, and let \(o_{m-1},o_m\) be the root's output times.

By \cref{lem:mature}, player \(j\), born at \(b_j\), outputs at local ages \(a_{j,r}=o_r+2(j-1)-b_j\) for \(r=m-1,m\). Actual adjacency gives the old register \(\ell_j=a_{j,m-1}\), so the update uses
\[
  a_{j,m}-\ell_j=o_m-o_{m-1},\qquad
  L_m=F(o_m-o_{m-1}).
\]
Thus the replay lengths agree, while the global deadlines retain the output offsets:
\begin{equation}
  Q_{j,m}=o_m+2(j-1)+L_m.
  \label{eq:common-wait-deadlines}
\end{equation}

\begin{sublemma}[Bounded maintenance under a general waiting rule]
\label{lem:maintenance}
Suppose two mature executions in a fixed nonempty market give consecutive actual outputs for every player, and the population remains fixed thereafter. Every subsequent maintenance cycle produces each player's next actual output in a mature execution, preserving the output offsets and a common waiting length. For cycle \(m\), let \(o=o_m\) and \(L=L_m\) be the current root output time and common waiting length, and put \(Q=o+L\). If \(o'\) is the next root output and \(V'\) its handoff completion round, then
\[
  0<C_m:=o'-Q\le2J+2K-1,\qquad
  V'-Q\le U=2K^2+14K,
\]
and
\[
  L_{\mathrm{next}}=F(L+C_m)\ge H+2(L+C_m)>2L.
\]
The maintenance window is \([Q,V')\); between these windows, \(M_t=m^*\).
\end{sublemma}

\begin{proof}[Proof of \cref{lem:maintenance,lem:known-maintenance}]
We induct on calibrated handoffs. The deadlines are \(Q+2(j-1)\) by \eqref{eq:common-wait-deadlines}, and \(L\ge H>2K\) places \(Q\) after the current handoff. Correct replay lasts until \(Q\); every other current replay ends by \(Q+2K-2\), possibly earlier after rejection. Once the root scans, \cref{lem:sweep}(i) excludes other work, scans, and outputs.

\emph{If \(m^*(1)\ne\BUS\)}, the root enters fresh \SEEK{} at \(Q\) with \(\rho=0\) and its rejection record cleared. Its \(J\) BUS acceptances in \(Q,\ldots,Q+J-1\) cannot trigger its own AA handoff and prevent every other AA start. Any other BUS replayer is rejected at \(Q\), before its own deadline, resetting its counter; non-BUS replayers already have zero counters. Thus no competing scan or work begins. Since \(J>2K-2\), all others are seekers when the root starts scanning at \(Q+J\), and the first block succeeds:
\begin{equation}
  c=Q+J+2K.
  \label{eq:maintenance-nonbus-entry}
\end{equation}

\emph{If \(m^*(1)=\BUS\)}, all \(L\ge H>J\) proposals in \(o,\ldots,Q-1\), including the output round \(o\), are accepted at BUS. The counter is saturated, so expiration followed by qualification starts \SWEEP{} at \(Q\). All other replays end by \(Q+2K-2\), so the second block, starting at \(Q+2K\), succeeds unless the first already did. Hence
\begin{equation}
  c\le Q+4K\le Q+J+2K.
  \label{eq:maintenance-bus-entry}
\end{equation}

In both cases, no output occurs between the current handoff and \(c\), and \(c\le Q+J+2K\). By \cref{lem:sweep}(ii) and \cref{lem:mature}, the next execution is mature and gives each player's next actual output with the same offsets. Since \(o'=c+J-1\),
\begin{equation}
  C_m:=o'-Q,\qquad 0<C_m\le2J+2K-1.
  \label{eq:maintenance-overhead}
\end{equation}
Calibration therefore applies again with \(o'-o=L+C_m\):
\begin{equation}
  L_{\mathrm{next}}=F(L+C_m)\ge H+2(L+C_m)>2L.
  \label{eq:wait-doubling}
\end{equation}

The last player enters \REPLAY{} one round after its output, so \(V'=o'+2(n-1)+1\le o'+2K-1\), giving
\begin{equation}
  V'-Q\le C_m+2K-1\le2J+4K-2=2K^2+14K=U.
  \label{eq:maintenance-window-budget}
\end{equation}
Thus \([Q,V')\) costs at most \(U\) mismatch rounds. Since \(L_{\mathrm{next}}\ge H>2K\), the next deadline follows \(V'\), with correct replay between the windows, completing the induction. Finally, \(L_0\ge H\), and monotonicity gives \(L_{\mathrm{next}}=F(L+C_m)\ge F(L)\). Applied to the pair supplied by \cref{lem:recovery}, these bounds prove \cref{lem:known-maintenance}.
\end{proof}


% \subsection{Calibration and bounded maintenance}
% \label{sec:proof-maintenance}

% \paragraph{Calibration from actual consecutive outputs.}
% Consider two mature executions in the same fixed market, consecutive in every player's actual output sequence. Label players by decreasing BUS preference, write \(m^*\) for the POSM, and let \(o_{m-1},o_m\) be the root's output times.

% \begin{proof}[Proof of the calibration identity]
% By \cref{lem:mature}, player \(j\), born at \(b_j\), outputs at local ages \(a_{j,r}=o_r+2(j-1)-b_j\) for \(r=m-1,m\). Actual adjacency, obtained initially from \cref{lem:recovery}, gives the old register \(\ell_j=a_{j,m-1}\). Before this register is overwritten, the local update satisfies
% \[
%   a_{j,m}-\ell_j=o_m-o_{m-1},\qquad
%   L_m=F(o_m-o_{m-1}).
% \]
% This common length gives global deadlines
% \begin{equation}
%   Q_{j,m}=o_m+2(j-1)+L_m,
%   \label{eq:common-wait-deadlines}
% \end{equation}
% preserving the output offsets.
% \end{proof}

% \begin{sublemma}[Bounded maintenance under a general waiting rule]
% \label{lem:maintenance}
% Suppose two actual consecutive mature executions occur in the same fixed nonempty market, and the population remains fixed thereafter. Every subsequent maintenance cycle produces each player's next actual output in a mature execution, preserving the fixed output offsets and a common waiting length. Let \(o\) and \(L\) be the current root output time and common waiting length, and let \(Q=o+L\). If \(o'\) is the next root output and \(V'\) the completion round of its handoff, then
% \[
%   0<C_m:=o'-Q\le2J+2K-1,\qquad
%   V'-Q\le U=2K^2+14K,
% \]
% and
% \[
%   L_{\mathrm{next}}=F(L+C_m)\ge H+2(L+C_m)>2L.
% \]
% The maintenance window is \([Q,V')\); between these windows, \(M_t=m^*\).
% \end{sublemma}

% \begin{proof}[Proof of \cref{lem:maintenance,lem:known-maintenance}]
% The computations supplied by \cref{lem:known-recovery} are mature, as established in \cref{sec:proof-recovery}, so it suffices to prove the stronger statement above. We induct on calibrated handoffs. The deadlines are \(Q+2(j-1)\) by \eqref{eq:common-wait-deadlines}, and \(L\ge H>2K\) places \(Q\) after the current handoff. Correct replay lasts until the root returns at \(Q\); each other current replay ends by \(Q+2K-2\), possibly earlier after rejection. Once the root scans, \cref{lem:sweep}(i) excludes other work, scans, and outputs.

% \emph{If \(m^*(1)\ne\BUS\)}, the root has \(\rho=0\) at \(Q\) and enters fresh \SEEK{} with its rejection record cleared. Its \(J\) BUS acceptances in \(Q,\ldots,Q+J-1\) cannot trigger its own AA handoff and prevent every other AA start. Any other BUS replayer is rejected at \(Q\), before its own deadline, resetting its counter; non-BUS replayers already have zero counters. Thus no competing scan or work begins. Since \(J>2K-2\), all other players are seekers when the root starts scanning at \(Q+J\), and the first block succeeds. Hence
% \begin{equation}
%   c=Q+J+2K.
%   \label{eq:maintenance-nonbus-entry}
% \end{equation}

% \emph{If \(m^*(1)=\BUS\)}, the \(L\ge H>J\) proposals in \(o,\ldots,Q-1\), including the output round \(o\), are accepted at BUS. The counter is saturated, so expiration followed by qualification starts \SWEEP{} in the same round \(Q\). All other replays end by \(Q+2K-2\), so the second block, starting at \(Q+2K\), succeeds unless the first already did. Thus
% \begin{equation}
%   c\le Q+4K\le Q+J+2K.
%   \label{eq:maintenance-bus-entry}
% \end{equation}

% Neither case permits an output between the current handoff and \(c\). The next execution is mature by \cref{lem:sweep}(ii), and \cref{lem:mature} gives each player's next actual output, with the same offsets. Since \(o'=c+J-1\),
% \begin{equation}
%   C_m:=o'-Q,\qquad 0<C_m\le2J+2K-1=:\overline C.
%   \label{eq:maintenance-overhead}
% \end{equation}
% The two outputs are actually adjacent, so calibration applies again with \(o'-o=L+C_m\):
% \begin{equation}
%   L_{\mathrm{next}}=F(L+C_m)\ge H+2(L+C_m)>2L.
%   \label{eq:wait-doubling}
% \end{equation}

% Finally, \(V'=o'+2(n-1)+1\le o'+2K-1\), giving
% \begin{equation}
%   V'-Q\le C_m+2K-1\le2J+4K-2=2K^2+14K=U.
%   \label{eq:maintenance-window-budget}
% \end{equation}
% Each physical round costs at most one in \(D\), so \([Q,V')\) costs at most \(U\). Since \(L_{\mathrm{next}}\ge H>2K\), the next deadline follows \(V'\), with correct replay between the windows. This preserves the induction. Finally, \(L_0\ge H\) follows from the waiting-rule condition, and monotonicity gives \(L_{\mathrm{next}}=F(L+C_m)\ge F(L)\); together with the uniform bound \(U=O(K^2)\), these are the claims of \cref{lem:known-maintenance}.
% \end{proof}



==> appendices/tradeoffs/mature-executions.tex <==
\subsection{Mature executions compute the POSM}
\label{sec:proof-mature}

Fix a nonempty market of \(n\le K\) players, labeled \(1,\ldots,n\) in decreasing BUS preference. Player \(1\) is the root, and \(m^*\) is the market's POSM. These labels and global round numbers are used only for analysis; players need not know their BUS ranks or detect the mature-entry condition below.

\begin{definition}[Mature entry]
\label{def:mature}
After the round-start updates in round \(c\) and before proposals, suppose the root has just entered \WORK{}, while every other player is in \SEEK{} with \(\rho=0\) and a BUS rejection recorded during its current \SEEK{} visit. Then \(c\) is a \emph{mature entry}, and the computation it initiates is a \emph{mature execution}.
\end{definition}

\begin{sublemma}[Mature work computes the POSM and fixes output offsets]
\label{lem:mature}
Suppose \(c\) is a mature entry and no population event occurs from \(c\) through \(V=c+J+2(n-1)\). Player \(j\) starts \WORK{} and outputs at
\[
  s_j=c+2(j-1),\qquad o_j=c+J-1+2(j-1)=o_1+2(j-1).
\]
The actual matching reaches \(m^*\) by \(c+J-2\) and remains there through \(V=o_n+1\le c+J+2K-2\). Each player outputs \(m^*(j)\) exactly once in \([c,V]\) and enters \REPLAY{} with that saved arm by \(V\).
\end{sublemma}

\begin{proof}[Proof of \cref{lem:mature}]
\emph{Entry and output times.}
At mature entry, each remaining seeker has a recorded BUS rejection and \(\rho=0\). While earlier entrants stay in \phase{Park}, the highest-priority remaining seeker receives two consecutive BUS acceptances and enters \WORK{} next round. Induction gives
\begin{equation}
  s_j=c+2(j-1),\qquad 1\le j\le n.
  \label{eq:mature-starts}
\end{equation}
For \(n\ge2\), the last qualifying pair ends at \(c+2n-3\le c+2K-3\), before the root leaves \phase{Park} at \(c+2K\). Each seeker takes its AA handoff before accumulating the \(J>2\) acceptances needed for a sweep. The case \(n=1\) is immediate.

The last entrant reaches \phase{Top} at \(t_0=c+2(n-1)+2K\le c+4K-2\), while the root remains in \phase{Top} through \(c+4K\). Thus all players are in \phase{Top} with application index \(1\) at \(t_0\). Since each \WORK{} invocation lasts exactly \(J\) rounds,
\begin{equation}
  o_j=s_j+J-1=o_1+2(j-1),
  \qquad o_1=c+J-1.
  \label{eq:mature-outputs}
\end{equation}
All players remain in \phase{Top} or \phase{DA} on \([t_0,o_1)\). By \cref{lem:top-da}, proved below, the matching reaches \(m^*\) by \(c+J-2<o_1\) and remains correct before the first output.

\emph{Output and replay.}
Every output assigns a replay length at least \(H\), so each new global deadline is at least \(o_j+H\ge o_1+H\). Since
\[
  V=o_n+1=o_1+2(n-1)+1\le o_1+2K-1<o_1+H,
\]
no replay expires during the handoff. Inductively, players still in \WORK{} repeat their accepted arms and save them at output, while players already in \REPLAY{} propose to those same arms and remain accepted. Hence the matching stays at \(m^*\) through \(V\). Each player outputs exactly once, enters \REPLAY{} at \(o_j+1\), and remains there through \(V\).
\end{proof}

The following lemma establishes the matching correctness used above.

\begin{sublemma}[\phase{Top} and \phase{DA} implement deferred acceptance with delays]
\label{lem:top-da}
Suppose player \(j\) starts \WORK{} at \(s_j=c+2(j-1)\), no population event occurs in \([c,o_1)\), where \(o_1=c+J-1\), and all players are in \phase{Top} with application index \(1\) at \(t_0=\max_j s_j+2K\). On \([t_0,o_1)\), the execution implements player-proposing deferred acceptance with delayed proposals. Every rejection processed in \phase{DA} excludes its edge from every stable matching. An arm that rejects a player retains an acceptor preferred to that player through round \(o_1-1\). An all-accepted round occurs by \(c+J-2\); its matching is \(m^*\) and persists through round \(o_1-1\).
\end{sublemma}

\begin{proof}
Call a rejection \emph{adopted} when it is processed in a nonfinal \phase{DA} round. On consecutive rounds of \([t_0,o_1)\), every accepted player repeats its arm, including across the \phase{Top}--\phase{DA} transition. If displaced, it is replaced by a proposer the arm prefers. Thus an arm's acceptor can only improve after its first acceptance in this interval.

For rejection validity, induct on rounds from \(t_0\), when all application indices are \(1\). Suppose \(i\) adopts a rejection at \(x\), whose winner is \(w\). Every arm that \(w\) prefers to \(x\) was passed after an adopted rejection in a strictly earlier round; this set is empty if \(w\) is still in \phase{Top}. By induction, none can be \(w\)'s partner in a stable matching \(m\). If \(m(i)=x\), then \(w\) prefers \(x\) to \(m(w)\), and \(x\) prefers \(w\) to \(i\), so \((w,x)\) blocks \(m\). This contradiction uses only rejections from earlier rounds.

A rejection at a player's last arm would require better actual acceptors at all \(K\) arms, by persistence at its previously rejected arms. These would be \(K\) distinct other players, contradicting \(n\le K\). Hence the cap never prevents an advance, and at most \(n(K-1)\) advances occur. Suppressing repeated proposals and processing each round's new proposals in any order gives a player-proposing DA execution with the same tentative matches at each round end; rejections during \phase{Top} delay subsequent proposals.

All players are in \phase{DA} by \(t_1=c+6K-1\), and
\begin{equation}
  t_1+n(K-1)
  \le c+6K-1+K(K-1)
  =c+J-2<o_1.
  \label{eq:mature-solve-time}
\end{equation}
Every round in \([t_1,t_1+n(K-1)]\) without universal acceptance produces an advance. These \(n(K-1)+1\) rounds therefore include an all-accepted round.

Let \(M\) be the matching in an all-accepted round. Every arm that a player prefers to its partner has rejected that player and retains a better acceptor, so \(M\) is stable. Rejection validity also excludes every such preferred edge from all stable matchings, proving \(M=m^*\). Repeated accepted proposals preserve this matching through round \(o_1-1\).
\end{proof}

The next two subsections establish mature entry from general reachable histories.



% \subsection{Mature executions compute the POSM}
% \label{sec:proof-mature}

% We first prove a conditional statement about a fixed, nonempty market. Fix \(1\le n\le K\) players, and label them \(1,\ldots,n\) in decreasing order of the preference of \(\BUS\). Call player \(1\) the root, and write \(m^*\) for this market's POSM. These labels, the root, and all global round numbers in this subsection are used only in the proof. Players neither know their BUS ranks nor test whether an execution satisfies the mature-entry conditions in \cref{def:mature}.

% \begin{definition}[Mature entry]
% \label{def:mature}
% Consider a round \(c\) with \(n\ge1\) players, labeled in decreasing priority at \(\BUS\). After round-start state updates and before proposals, suppose player \(1\) has just entered \WORK{}, while every other player is in \SEEK{} with \(\rho=0\) and a BUS rejection recorded during its current \SEEK{} visit. Then \(c\) is a \emph{mature entry}, and the computation it initiates is a \emph{mature execution}.
% \end{definition}

% \begin{sublemma}[Mature work computes the POSM and fixes output offsets]
% \label{lem:mature}
% Suppose \(c\) is a mature entry and no population event occurs through \(V=c+J+2(n-1)\). Player \(j\) starts \WORK{} and outputs at
% \[
%   s_j=c+2(j-1),\qquad o_j=c+J-1+2(j-1)=o_1+2(j-1).
% \]
% The actual matching reaches \(m^*\) by \(c+J-2\) and remains there through \(V=o_n+1\le c+J+2K-2\). Each player outputs \(m^*(j)\) exactly once in \([c,V]\) and enters \REPLAY{} with that saved arm by \(V\).
% \end{sublemma}

% \input{figures/mature-execution}

% Reaching the POSM, saving an output, and entering \(\REPLAY\) refer to three different points in the execution. We first analyze the matching procedure before any output, then verify its entry conditions and the handoff to replay.

% \begin{sublemma}[\phase{Top} and \phase{DA} implement deferred acceptance with delays]
% \label{lem:top-da}
% In the fixed market above, suppose no population event occurs from \(c\) through \(c+J-2\), player \(j\) starts \(\WORK\) at \(s_j=c+2(j-1)\), and all players are in \phase{Top} with DA application index \(1\) at \(t_0=\max_j s_j+2K\). From \(t_0\) until the first output round \(o_1=c+J-1\), the execution implements player-proposing Gale--Shapley deferred acceptance in which rejected players may delay their next proposals. Every adopted rejection excludes its edge from every stable matching. An arm that rejects a player has an actual acceptor preferred to that player in that round and every subsequent round before \(o_1\). An all-accepted round occurs by \(c+J-2\); its matching is \(m^*\) and persists until the first output.
% \end{sublemma}

% \begin{proof}
% Call a rejection \emph{adopted} when it is processed in a nonfinal \phase{DA} round. On consecutive rounds of the stated interval, an accepted player repeats its arm, including across the transition from \phase{Top} to \phase{DA}. If displaced, it is replaced by a proposer the arm prefers. Thus every arm that acquires an actual acceptor retains one whose rank can only improve. Repeated proposals maintain these tentative matches, with each arm choosing its most-preferred current proposer in every round.

% Induct on rounds to prove rejection validity, starting with all application indices equal to \(1\) at \(t_0\). Suppose \(i\) adopts a rejection at \(x\), whose actual winner is \(w\). Every arm that \(w\) prefers to \(x\) was passed after an adopted rejection in a strictly earlier round; there are no such arms if \(w\) is still in \phase{Top}. By induction, none can be \(w\)'s partner in a stable matching \(m\). If \(m(i)=x\), then \(m(w)\ne x\), so \(w\) prefers \(x\) to \(m(w)\), including when unmatched. Since \(x\) prefers \(w\) to \(i\), the pair \((w,x)\) blocks \(m\), a contradiction. This argument uses no rejection from the current round.

% A rejection at a player's last arm would require better actual acceptors at all \(K\) arms, by persistence at its previously rejected arms. Since each player makes one proposal per round, these would be \(K\) distinct other players, contradicting \(n\le K\). Hence the cap never prevents an advance, and at most \(n(K-1)\) advances occur. Suppressing repeated proposals and processing each round's new proposals in any order now gives a GS execution with the same tentative matches at every round end. Rejections during \phase{Top} delay the next GS proposal; real players still make one proposal per physical round.

% All players are in \phase{DA} by \(t_1=c+(2K-2)+(4K+1)=c+6K-1\), and
% \begin{equation}
%   t_1+n(K-1)
%   \le c+6K-1+K(K-1)
%   =c+J-2<o_1.
%   \label{eq:mature-solve-time}
% \end{equation}
% Every non-all-accepted round in this interval produces an advance. Its \(n(K-1)+1\) rounds therefore include an all-accepted round.

% Let \(M\) be the matching in such a round. Any arm that \(i\) prefers to \(M(i)\) has rejected \(i\) and retains a better acceptor, so \(M\) is stable. Rejection validity also excludes those preferred arms as \(i\)'s partner in every stable matching, proving \(M=m^*\). Each player then repeats its accepted arm, preserving the matching until the first output.
% \end{proof}

% \begin{proof}[Proof of \cref{lem:mature}]
% At mature entry, the root starts \WORK{} and every other player seeks BUS with a recorded rejection and \(\rho=0\). The highest-priority remaining seeker receives two consecutive acceptances while earlier entrants stay in \phase{Park}, off BUS; lower-priority seekers are rejected. Induction gives
% \begin{equation}
%   s_j=c+2(j-1),\qquad 1\le j\le n.
%   \label{eq:mature-starts}
% \end{equation}
% For \(n\ge2\), the last qualifying pair ends at \(c+2n-3\le c+2K-3\), before the root leaves \phase{Park} at \(c+2K\); later entrants leave still later. Each seeker takes its AA handoff after only two consecutive acceptances, before qualifying for a scan. For \(n=1\), the start-time claim is immediate.

% The last entrant reaches \phase{Top} at
% \[
%   t_0=c+2(n-1)+2K\le c+4K-2.
% \]
% The root remains in \phase{Top} through \(c+4K\), so at \(t_0\) all players are in \phase{Top} with application index \(1\). Each \WORK{} invocation lasts exactly \(J\) rounds regardless of feedback, giving
% \begin{equation}
%   o_j=s_j+J-1=o_1+2(j-1),
%   \qquad o_1=c+J-1.
%   \label{eq:mature-outputs}
% \end{equation}
% All players stay in \phase{Top} or \phase{DA} from \(t_0\) until \(o_1\). Thus \cref{lem:top-da} applies and the actual matching reaches \(m^*\) by \(c+J-2<o_1\), without requiring players to detect this event.

% At \(o_j\), the old output age satisfies \(\ell_j\le a_j\), since it is initialized to zero and updated only at outputs. Using \(H>2K\), the new deadline and the last replay-entry round satisfy
% \[
% \begin{aligned}
%   b_j+q_j&=o_j+F(a_j-\ell_j)\ge o_1+H,\\
%   V=o_n+1&=o_1+2(n-1)+1\le o_1+2K-1<o_1+H.
% \end{aligned}
% \]
% Thus no new replay deadline expires by \(V\). Starting from \(m^*\) before \(o_1\), induction over the handoff rounds shows that players still in \WORK{} repeat their accepted arms and save them at output, while players in \REPLAY{} propose to the same arms, are accepted, and have unexpired deadlines. With no population event, the matching therefore remains \(m^*\) through \(V\). Every player outputs \(m^*(j)\) exactly once, enters \REPLAY{} at \(o_j+1\), and never returns to \SEEK{} during the handoff.
% \end{proof}

% The next two subsections establish mature entry from general reachable histories.


==> appendices/tradeoffs/recovery.tex <==
\subsection{Recovery to consecutive mature executions}
\label{sec:proof-recovery}

The waiting rule \(F\) satisfies \eqref{eq:general-wait-condition}. Define the nondecreasing recovery map
\begin{equation}
 \Psi_F(x)=x+F(x+H)+3H.
 \label{eq:general-recovery-map}
\end{equation}

\begin{sublemma}[Recovery to actual consecutive mature outputs]
\label{lem:recovery}
For every normally initialized finite-event history with a nonempty final market, two mature handoffs beginning after \(t_*\) complete by a round
\begin{equation}
 V_{\mathrm{cal}}\le\Psi_F^{\circ3}(t_*+1).
 \label{eq:recovery-time}
\end{equation}
Each player's two outputs are consecutive in its actual output history, so the second output uses the local age of the first as its old \(\ell\).
\end{sublemma}

\begin{proof}[Proof of \cref{lem:recovery,lem:known-recovery}]
Let \(n\) be the final population size and \(z\) its highest-priority player at BUS. States are taken after round-start updates. At any output in round \(v\), including an incorrect one, a player born at \(b_i\ge1\) has \(0\le\ell\le a=v-b_i\le v\). By monotonicity of \(F\), the old register \(\ell\) gives the global deadline
\begin{equation}
 Q_i=v+F(a-\ell)\le v+F(v).
 \label{eq:replay-deadline-bound}
\end{equation}
Replay expires in its deadline round; acceptance never extends it, and rejection can end it earlier.

\paragraph{First mature handoff.}
From round \(t_*+1\), \(z\) is never rejected at BUS. Before reaching a continuing scan, it can produce at most one output from inherited work or an old seek rejection record, and any such output occurs by \(t_*+J+2\). A fresh seek clears that record and cannot trigger an AA handoff. By \eqref{eq:replay-deadline-bound}, every preceding replay ends by \(t_*+J+2+F(t_*+J+2)\). At most \(J\) further qualification rounds therefore give a continuing scan by
\begin{equation}
 \beta\le t_*+J+2+F(t_*+J+2)+J
 \le\Psi_F(t_*+1).
 \label{eq:continuing-scan-time}
\end{equation}
An inherited scan already satisfies the isolation invariant from its original qualified entry, even if events occurred in the meantime.

Until success, \cref{lem:sweep}(i) excludes other work, scans, and outputs. All remaining replays therefore expire by \(\beta+F(\beta)\). A residual block and one full block take at most \(4K\) further rounds; the full block succeeds if no earlier one does. By \cref{lem:sweep,lem:mature}, the resulting mature handoff completes at
\begin{equation}
 V_{\mathrm{first}}
 \le\beta+F(\beta)+J+6K-2\le\Psi_F(\beta).
 \label{eq:first-recovery-handoff}
\end{equation}
All players are then in correct \REPLAY{}, although their waiting lengths can differ.

\paragraph{The next work start is mature.}
Before any new work starts, no output replaces the current deadlines, all of which are at most \(V_{\mathrm{first}}+F(V_{\mathrm{first}})\). If no work has started by that round, all current replays have ended. Player \(z\) is then already scanning or qualifies within \(J\) rounds, and a residual block followed by a full block succeeds within at most \(4K\) more rounds. Thus a new work start exists by \(V_{\mathrm{first}}+F(V_{\mathrm{first}})+J+4K\); let \(r\) be the first such start.

Suppose player \(i\) starts through an AA handoff. Its current seek visit began after \(V_{\mathrm{first}}\) with the rejection flag cleared. The final acceptance run must have length exactly two, or work would have started earlier. Hence, in that same visit, \(i\) was rejected at \(r-3\) and accepted at \(r-2,r-1\).

Let \(w\) be the BUS winner at \(r-3\). It outranks \(i\) and remains present, so it must avoid BUS in both following rounds. A winning seeker continues on BUS, including upon scan qualification; a player accepted while replaying BUS proposes there again, including after expiration; and a continuing scan leaves BUS only for isolated rounds. A work entry in either intervening round would contradict the choice of \(r\). This two-round absence is impossible, so the first new work follows a successful scan and is mature by \cref{lem:sweep}(ii).

\paragraph{Consecutive outputs and calibration.}
By \cref{lem:mature}, each player outputs exactly once in each mature execution. No output occurs between the first handoff and \(r\), so these are consecutive actual outputs. The bound on \(r\), followed by \(J+2(n-1)\) handoff rounds, gives
\begin{equation}
 \begin{aligned}
 V_{\mathrm{cal}}
 &\le V_{\mathrm{first}}+F(V_{\mathrm{first}})+2J+6K-2\\
 &\le\Psi_F(V_{\mathrm{first}})
 \le\Psi_F^{\circ3}(t_*+1).
 \end{aligned}
 \label{eq:second-recovery-handoff}
\end{equation}
For \(K\ge2\), \(J+1<H\), \(J+6K-2<H\), and \(2J+6K-2<H\); these inequalities and monotonicity justify all three applications of \(\Psi_F\).

The two mature executions have the same player offsets. Their actual adjacency therefore makes every player's output-age difference equal to the root's inter-output duration. Applying \(F\) gives a common replay length at the second handoff, with staggered deadlines as detailed in \cref{sec:proof-maintenance}. Together with matching correctness, this proves \cref{lem:known-recovery}.
\end{proof}


% \subsection{Recovery to consecutive mature executions}
% \label{sec:proof-recovery}

% The waiting rule \(F\) satisfies \eqref{eq:general-wait-condition}. Define the nondecreasing recovery map
% \begin{equation}
%  \Psi_F(x)=x+F(x+H)+3H.
%  \label{eq:general-recovery-map}
% \end{equation}

% \begin{sublemma}[Recovery to actual consecutive mature outputs]
% \label{lem:recovery}
% For every normally initialized finite-event history with a nonempty final market, two mature handoffs beginning after \(t_*\) complete by a round
% \begin{equation}
%  V_{\mathrm{cal}}\le\Psi_F^{\circ3}(t_*+1).
%  \label{eq:recovery-time}
% \end{equation}
% Their outputs are consecutive in each player's actual output history. Thus, immediately before its second output updates \(\ell\), the register still holds the local age of its first output.
% \end{sublemma}

% \begin{proof}[Proof of \cref{lem:recovery,lem:known-recovery}]
% Let \(n\) be the final population size and \(z\) its highest-priority player at BUS. All states are taken after round-start updates. At an actual output in global round \(v\), a player born at \(b_i\ge1\) has \(0\le\ell\le a=v-b_i\le v\). Monotonicity gives
% \begin{equation}
%  Q_i=v+F(a-\ell)\le v+F(v).
%  \label{eq:replay-deadline-bound}
% \end{equation}
% This bound includes incorrect outputs. Expiration acts in the deadline round; acceptance does not extend the deadline, and rejection can end replay earlier.

% \paragraph{First mature handoff.}
% From round \(t_*+1\), player \(z\) is never rejected at BUS. An inherited work invocation or a seeker with an old rejection record produces at most one output before a fresh seek, by \(t_*+J+2\). A fresh seek clears that record. An inherited replay comes from an earlier output; an inherited scan may continue. Once replay ends, at most \(J\) BUS acceptances give scan qualification. Thus \(z\) reaches a continuing qualified scan by
% \begin{equation}
%  \beta\le t_*+J+2+F(t_*+J+2)+J
%  \le\Psi_F(t_*+1).
%  \label{eq:continuing-scan-time}
% \end{equation}
% An inherited scan retains the isolation invariant from its original qualified entry, even if events occurred in the meantime.

% Until the scan succeeds, \cref{lem:sweep}(i) excludes other work, scans, and outputs. Every remaining replay therefore comes from an output before \(\beta\), and expires by \(\beta+F(\beta)\). Unless success occurs sooner, a residual block and one full block take at most \(4K\) further rounds. The full block succeeds and \cref{lem:sweep,lem:mature} give a mature handoff at
% \begin{equation}
%  V_{\mathrm{first}}
%  \le\beta+F(\beta)+J+6K-2\le\Psi_F(\beta).
%  \label{eq:first-recovery-handoff}
% \end{equation}
% All players are then in correct \REPLAY{}, although their waiting lengths can differ.

% \paragraph{Actual adjacency of the outputs.}
% Consider the first actual work start \(r>V_{\mathrm{first}}\), whose existence is established below. If player \(i\) starts through an AA handoff, its current seek visit began after \(V_{\mathrm{first}}\) with the rejection flag cleared. The acceptances in rounds \(r-2,r-1\) therefore require a rejection at \(r-3\): an acceptance there would either leave the flag clear or have triggered an earlier work start.

% Let \(w\) be the BUS winner at \(r-3\). It outranks \(i\) and remains present, so it must avoid BUS in both \(r-2\) and \(r-1\). No player is in work between the first handoff and \(r\). A winning seeker continues on BUS, including when it qualifies to scan. A player accepted while replaying BUS proposes there again next round, including after expiration. A continuing scan leaves BUS only for isolated rounds. A scheduled work entry in either intervening round would contradict the minimality of \(r\). The required two-round absence is therefore impossible.

% Consequently the first new work follows a successful scan and is mature. \Cref{lem:mature} excludes extra outputs between a player's first mature output and the first handoff; there is no output before the next work starts; and that mature execution gives exactly one new output per player. The two outputs are actual neighbors in each player's history.

% \paragraph{Time of the second handoff.}
% Until that next work starts, no output replaces the deadlines, which are all at most \(V_{\mathrm{first}}+F(V_{\mathrm{first}})\). Once these deadlines expire, \(J\) qualification rounds, at most \(4K\) scan rounds, and \(J+2(n-1)\) handoff rounds suffice. Thus the first new work does exist, and this very next mature handoff satisfies
% \begin{equation}
%  \begin{aligned}
%  V_{\mathrm{cal}}
%  &\le V_{\mathrm{first}}+F(V_{\mathrm{first}})+2J+6K-2\\
%  &\le\Psi_F(V_{\mathrm{first}})
%  \le\Psi_F^{\circ3}(t_*+1).
%  \end{aligned}
%  \label{eq:second-recovery-handoff}
% \end{equation}
% For \(K\ge2\), \(J+1<H\), \(J+6K-2<H\), and \(2J+6K-2<H\); these inequalities and monotonicity justify the three recovery steps. No free reset or arbitrary-state initialization is used.

% Both computations are mature, so \cref{lem:mature} gives correct outputs with the same player offsets. Actual adjacency makes the difference between each player's current output age and its old \(\ell\) equal to the root's inter-output duration. Applying \(F\) therefore gives a common replay length at the second handoff, while the deadlines retain the output offsets, as detailed in \cref{sec:proof-maintenance}. This proves \cref{lem:known-recovery}.
% \end{proof}


==> appendices/tradeoffs/scda-interface.tex <==
\subsection{SC-DA with a general local waiting rule}
\label{sec:tradeoff-native-interface}

The upper bound uses the recovery and maintenance lemmas through the following accounting statement. It bounds the total cost by the calibration prefix and the number of maintenance windows.

Use \(J,H\) from \eqref{eq:parameters} and \(U=2K^2+14K\) from \eqref{eq:maintenance-window-budget}. Fix a nondecreasing computable \(F:\mathbb N_{\ge1}\to\mathbb N_{\ge1}\) satisfying \eqref{eq:general-wait-condition}, and use the update \eqref{eq:general-wait-update}. Define
\[
 b_0=H,\qquad b_{j+1}=F(b_j),\qquad
 N_F(T)=\#\{j\ge0:b_j<T\}.
\]
This auxiliary count is distinct from the budget count \(N_g\).

\begin{sublemma}[Recovery and maintenance under a local waiting rule]
\label{lem:general-wait-interface}
For every normally initialized finite-event history with a nonempty final market, two mature handoffs with actual consecutive outputs complete by
\[
 V_{\mathrm{cal}}\le\Psi_F^{\circ3}(t_*+1).
\]
After this handoff, write \(o_j\) for the root output times and \(L_j\) for the common waiting lengths, starting with the second recovery output. If the final market has \(n\) players, put \(d_0=2n-1\), \(V_j=o_j+d_0\), and \(Q_j=o_j+L_j\). Then \(V_0=V_{\mathrm{cal}}\), and
\begin{align}
 o_{j+1}&=o_j+L_j+c_j,
 &0<c_j&\le2J+2K-1, \label{eq:general-output-recursion}\\
 L_{j+1}&=F(L_j+c_j)\ge H+2L_j,
 &V_{j+1}-Q_j&\le U. \label{eq:general-maintenance-recursion}
\end{align}
From \(V_{\mathrm{cal}}\) onward, matching is correct outside \([Q_j,V_{j+1})\). For all legal instances, including an empty final market, and every integer \(T\ge0\),
\begin{equation}
 D_F(T;I)\le
 \min\{T,\Psi_F^{\circ3}(t_*+1)+U N_F(T)\}.
 \label{eq:general-wait-accounting}
\end{equation}
\end{sublemma}

\begin{proof}
\emph{Calibration and maintenance.} \Cref{lem:recovery} supplies the two actual consecutive mature outputs. \Cref{sec:proof-maintenance} gives their common waiting length and \cref{lem:maintenance} supplies the recurrences, fixed output offsets, and correct replay outside maintenance windows. Both lemmas apply to the general waiting rule \(F\), independently of \cref{thm:known}.

\emph{Counting windows in a prefix.} Since \(L_0\ge H=b_0\) and \(L_{j+1}\ge F(L_j)\), monotonicity yields \(L_j\ge b_j\). A window meeting the evaluation prefix \(\{1,\ldots,T\}\) starts at \(Q_j\le T\). As \(o_j\ge1\),
\[
 b_j\le L_j=Q_j-o_j\le T-1<T.
\]
Thus at most \(N_F(T)\) windows can contribute, each costing at most \(U\), including an unfinished last window. Charging one per round before \(V_{\mathrm{cal}}\) proves the bound for prefixes reaching calibration.

Earlier prefixes satisfy \(D_F(T;I)\le T<V_{\mathrm{cal}}\). For an empty final market, no cost occurs from \(t_*\) onward, and \(D_F(T;I)\le\min\{T,t_*-1\}\). Finally \(D_F(0;I)=0\), so the accounting covers every horizon.
\end{proof}


==> appendices/tradeoffs/sweep-isolation.tex <==
\subsection{Successful sweeps establish mature entry}
\label{sec:proof-sweep}

The BUS qualification interval clears earlier computations, and the sweep's isolated one-round gaps at BUS prevent new ones from starting. This isolation holds before success and is used in the recovery proof. A successful block then brings all other players to \SEEK{} and establishes the mature entry required by \cref{lem:mature}.

\begin{sublemma}[Sweep isolation and mature entry]
\label{lem:sweep}
Consider a history of \protocol{} reachable from the prescribed initialization, and let player \(z\) enter \SWEEP{} in global round \(b\).
\begin{enumerate}[label=(\roman*)]
  \item \emph{Isolation during a continuing scan.} Suppose \(z\) remains in this visit through round \(d\) and is accepted at every BUS action in rounds \(b,\ldots,d\). At the start of \(b\), after all round-start checks, every other present player is in \SEEK{} or \REPLAY{}, with \(\rho=0\) and no pending \WORK{} entry. Throughout \(b,\ldots,d\), all other players remain in \SEEK{} or \REPLAY{} and never schedule \WORK{}; in particular, none enters \SWEEP{} or produces an output. Population events and failed blocks are allowed.
  \item \emph{Mature entry after success.} If this visit completes an all-accepted block in round \(e\), and no population event occurs in round \(c=e+1\), then \(c\) is a mature entry with \(z\) as root. Population events during qualification and the scan, including at the start of round \(e\), are allowed.
\end{enumerate}
\end{sublemma}

\begin{proof}
\emph{Clearing earlier computations.}
Round-start states are taken after population events, pending mode changes, expiration, and qualification. Put \(v=b-J\). Since every action other than an accepted BUS proposal resets \(\rho\), even after saturation, qualification at \(b\) implies that \(z\) is accepted at BUS in
\begin{equation}
  v,v+1,\ldots,b-1.
  \label{eq:sweep-qualification}
\end{equation}
No other player can complete an AA pair or a successful block in this interval, since both require a final BUS acceptance. Thus no other \WORK{} entry is scheduled.

Any \WORK{} entry pending from \(v-1\) takes effect at \(v\), so all earlier \WORK{} invocations finish by \(v+J-1=b-1\). A competing sweep present at \(v\) reaches BUS by \(v+1\) and, if still present, returns to \SEEK{} by \(v+2\). Every other player's counter is reset in each qualification round, excluding new sweeps in \(v+1,\ldots,b\). Since \(J>2\), all other players are in \SEEK{} or \REPLAY{} at \(b\), with zero counters and no pending \WORK{}. Arrivals start in \SEEK{} with \(\rho=0\), and departures simply remove players.

\emph{Isolation during the sweep.}
The scan word \eqref{eq:sweep} leaves BUS only for isolated single rounds, including across failed-block restarts. Non-BUS rejections mark a block as failed without restarting it. Since \(z\) wins every BUS action, every other player's consecutive BUS-acceptance count stays at most one. Thus neither an AA handoff nor a new sweep qualification is possible, and all other players remain in \SEEK{} or \REPLAY{}. This proves (i) on every continuing prefix, regardless of eventual success.

\emph{Mature entry after success.}
On a BUS rejection, the player skips the block-completion test and leaves \SWEEP{} in the following round. Thus a visit completing a successful block at \(e\) has only BUS acceptances, and (i) applies with \(d=e\). No other output occurs: each old replay keeps its saved arm until it ends, and no seeker reenters \REPLAY{}. A player still replaying when its saved arm is visited is rejected. Every arm is visited by \(e-2\), so all old replays have ended by \(e-1\); later arrivals start in \SEEK{}.

The final two proposals are to BUS. In round \(e\), every other present player, including any new arrival, therefore proposes to BUS and is rejected. Each ends the round in \SEEK{} with a rejection recorded during its current visit, \(\rho=0\), and no pending \WORK{}. Since \(z\) wins against all these players, it is the highest-ranked player at BUS. With no population event at \(c=e+1\), its scheduled \WORK{} entry establishes the mature entry in \cref{def:mature}.
\end{proof}



==> figures/mature-execution.tex <==
% !TeX root = ../main.tex
\begin{figure}[htbp]
\centering
\begin{tikzpicture}[x=0.48cm,y=1cm,line width=0.45pt]
  % The horizontal coordinate is the global round index minus c.
  \foreach \s/\y/\j in {0/3.3/1,2/2.2/2,4/1.1/3} {
    \draw[densely dotted] (0,\y) -- (\s,\y);
    \draw[fill=black!12] (\s,\y-0.25) rectangle (\s+6,\y+0.25);
    \draw[fill=black!4] (\s+6,\y-0.25) rectangle (\s+13,\y+0.25);
    \draw (\s+13,\y-0.25) rectangle (\s+25,\y+0.25);
    \draw[->] (\s+25,\y) -- (30,\y);
    \node[anchor=east] at (-0.6,\y) {\(j=\j\)};
  }
  \draw[dashed,black!55] (10,0.7) -- (10,3.8);
  \draw[dashed,black!55] (23,0.7) -- (23,3.8);
  \node[anchor=south] at (10,3.85) {common \phase{Top} round};
  \node[anchor=south] at (23,3.85) {POSM reached by};
  \foreach \s/\y/\j in {0/3.3/1,2/2.2/2,4/1.1/3} {
    \node at (\s+3,\y) {\phase{Park}};
    \node at (\s+18,\y) {\phase{DA}};
    \fill (\s+24,\y) circle (2pt);
    \node[anchor=north] at (\s+24,\y-0.31) {\(o_{\j}\)};
  }
  \node at (8.4,3.3) {\phase{Top}};
  \node at (11.5,2.2) {\phase{Top}};
  \node at (13.5,1.1) {\phase{Top}};
  \node[anchor=south] at (27.5,3.6) {\REPLAY{}};
  \draw[->] (0,0) -- (30.4,0);
  \foreach \t in {0,6,10,13,17,23,29} {
    \draw (\t,0.07) -- (\t,-0.07);
    \node[anchor=north] at (\t,-0.1) {\(\t\)};
  }
  \node[anchor=north] at (15,-0.55) {global round minus \(c\)};
\end{tikzpicture}
\caption{A mature execution with \(K=n=3\), hence \(J=25\).
Players are labeled by decreasing BUS preference. Their \WORK{} starts
are \(c,c+2,c+4\); the dotted lines before \WORK{} are \SEEK{}.
Each box covers the rounds of the indicated segment;
all players are in \phase{Top} at \(c+10\). The matching reaches the POSM by
\(c+23\), possibly earlier. Filled circles mark the output rounds
\(o_1=c+24\), \(o_2=c+26\), and \(o_3=c+28\). The lines after \WORK{}
are \REPLAY{}, starting in rounds \(c+25,c+27,c+29\), respectively.
Thus the matching is correct before the first output, and all players
have entered \REPLAY{} by \(c+29\). The timing is guaranteed by
\cref{lem:mature}; the diagram uses global time only for analysis.}
\label{fig:mature-timing}
\end{figure}


==> figures/scpc-work-timing.tex <==
\begin{figure}[p]
\definecolor{scpcnavy}{HTML}{264861}
\definecolor{scpclightblue}{HTML}{EAF1F6}
\definecolor{scpclightgreen}{HTML}{EDF3ED}
\definecolor{scpclightgray}{HTML}{F3F3F3}
\centering
\begin{tikzpicture}[>=latex,font=\small,x=1cm,y=1cm,
 labeltext/.style={align=center,font=\footnotesize},axis/.style={->,draw=scpcnavy,thick}]
\node[anchor=west,font=\bfseries] at (0,1.0) {(a) One player's work index $h$};
\fill[scpclightblue] (0,0) rectangle (2.15,.52);
\fill[scpclightgray] (2.15,0) rectangle (4.25,.52);
\fill[scpclightgreen] (4.25,0) rectangle (8.45,.52);
\fill[scpclightgray] (8.45,0) rectangle (11.6,.52);
\draw[axis] (0,0) -- (12.1,0);
\foreach \x/\txt in {0/0,2.15/d_L,4.25/h_{D,L},8.45/f_L,11.6/J_L-1}{
 \draw (\x,.58)--(\x,-.13);
 \node[below,font=\footnotesize] at (\x,-.15) {$\txt$};
}
\node[labeltext] at (1.07,.28) {Park};
\node[labeltext] at (3.2,.28) {Learn};
\node[labeltext] at (6.35,.28) {Learn and delete};
\node[labeltext] at (10.0,.28) {Continue requests};
\node[labeltext,text width=6.2cm] at (3.1,-1.15)
 {Certification is allowed through $h=f_L$.\\Deletion is allowed only for $h_{D,L}\le h<f_L$.};
\draw[->] (8.45,-.95)--(8.45,-.58);
\node[labeltext,text width=3.3cm] at (8.1,-1.65) {At $f_L$: last certificate.\\After $f_L$: no new certificate\\and no deletion.};
\draw[->] (11.6,-.95)--(11.6,-.58);
\node[labeltext,text width=2.4cm] at (11.2,-1.55) {At $J_L-1$:\\output after feedback.};
\node[anchor=west,font=\bfseries] at (0,-4.0) {(b) Overlapping work in a mature episode};
\draw[axis] (0,-5.0)--(12.1,-5.0);
\draw[scpcnavy,thick] (0,-4.7)--(10.4,-4.7);
\draw[scpcnavy,thick] (1.3,-5.3)--(11.7,-5.3);
\node[anchor=east,labeltext] at (-.08,-4.7) {root};
\node[anchor=east,labeltext] at (-.08,-5.3) {latest\\allowed};
\fill[scpclightgreen,opacity=.8] (4.1,-5.75) rectangle (8.75,-4.25);
\draw[densely dashed] (4.1,-5.9)--(4.1,-4.15);
\draw[densely dashed] (8.75,-5.9)--(8.75,-4.15);
\node[labeltext] at (6.425,-4.43) {$I_0$: every player can delete};
\node[labeltext] at (6.425,-5.54) {$|I_0|=f_L-\kappa_L-h_{D,L}=W_L$};
\node[labeltext,below] at (0,-5.85) {$c_0$};
\node[labeltext,below] at (1.3,-6.42) {$c_0+\kappa_L$};
\node[labeltext,below] at (4.1,-5.85) {$c_0+\kappa_L+h_{D,L}$};
\node[labeltext,below] at (8.75,-6.42) {$c_0+f_L$};
\node[labeltext,below] at (11.3,-5.85) {outputs, then\\common replay $S$};
\node[labeltext,text width=11.5cm] at (5.9,-7.65)
 {Each player's actual entry lies in $[c_0,c_0+\kappa_L]$.\\The minimum grace guarantees a common replay round before the next collection.};
\end{tikzpicture}
\caption{Work timing within one invocation and across a mature episode (schematic, not to scale). Panel (b) uses physical rounds: $c_0$ is the root's work-entry time, $c_i$ is player $i$'s entry time, and $S=\max_i(c_i+J_L)$ is the first common replay round. The shaded interval is $I_0=[c_0+\kappa_L+h_{D,L},c_0+f_L)\cap\mathbb Z$. The lower line represents an invocation beginning at the latest permitted time; the actual entry span may be smaller than $\kappa_L$. The action at index $h$ precedes that round's feedback. The final possible certification occurs no later than the earliest output round and precedes the output feedback in that round. Every $K$-rejection run that triggers a deletion occurs after all players have left parking and before the first output. The shaded interval is the common work window used to establish the sample quota for a failed good episode.}
\label{fig:scpc-work-timing}
\end{figure}


==> sections/04_trade-off_thm4_old_.tex <==
\section{Lower Bounds and Optimality}
\label{sec:lower-bounds}
\label{sec:tradeoffs}

Detecting an unannounced departure may require proposals that disrupt an otherwise correct matching. We formalize the resulting recovery requirement, establish the necessary mismatch cost, and characterize optimal static maintenance.
Throughout this section, we consider the known-preference setting, where each arm accepts its most preferred proposer in every round.

\subsection{Recovery and Necessary Mismatch}
\label{sec:tradeoff-problem}
\label{sec:tradeoff-bounds}

For a protocol \(\Pi\) and a legal finite-event instance \(I\) with last population-event time \(t_*\), define
\begin{equation}
 L_\Pi(h;I)=\mathbb E\!\left[D_\Pi(t_*+h;I)-D_\Pi(t_*;I)\right],
 \qquad h\ge1.
 \label{eq:recovery-window}
\end{equation}
This is the expected mismatch in rounds \(t_*+1,\ldots,t_*+h\), after the last population event. Players that remain active across the event retain their actual states.

\begin{definition}[Sublinear mismatch cost relative to \(g\)]
\label{def:sublinear-mismatch}
Let \(g:\mathbb N_{\ge1}\to\mathbb N_{\ge1}\) be nondecreasing. A decentralized matching protocol \(\Pi\) has \emph{sublinear mismatch cost relative to \(g\)} if, for every \(\varepsilon\in(0,1)\), there is a constant \(c_\varepsilon>0\) such that, for every legal finite-event instance \(I\) with last population-event time \(t_*\) and every \(h\ge c_\varepsilon g(t_*)\),
\[
 \frac{L_\Pi(h;I)}h\le\varepsilon.
\]
\end{definition}

The condition makes the expected post-event average mismatch arbitrarily small with a threshold uniform over instances, while allowing later maintenance. 
% Occasional maintenance mismatches may continue indefinitely. Here \(K,\Pi,g\) are fixed; \(c_\varepsilon\) may depend on them and on \(\varepsilon\), but not on the instance or the window length.
\begin{corollary}[Recovery of flexible SC-DA]
\label{cor:flexible-sublinear}
For every \(K\ge2\) and every nondecreasing, polynomial-time computable \(g:\mathbb N_{\ge1}\to\mathbb N_{\ge1}\) with \(g(t)=\Omega(t)\), the protocol \(\Pi_g\) in \Cref{thm:general-budget-upper} has sublinear mismatch cost relative to \(g\).
\end{corollary}

This follows by bounding recovery and subsequent maintenance within each post-event window; the proof is in \Cref{sec:tradeoff-upper-proof}. In particular, the original SC-DA satisfies the condition at the linear scale.

The lower bound requires only that \(g\) be a nondecreasing positive integer function. For such scales, use the same recurrence \eqref{eq:budget-iteration-count} to define \(N_g(T)\).

\begin{theorem}[Necessary mismatch cost]
\label{thm:recovery-maintenance}
For every \(K\ge2\), every nondecreasing \(g:\mathbb N_{\ge1}\to\mathbb N_{\ge1}\), and every legal randomized adaptive protocol \(\Pi\) with sublinear mismatch cost relative to \(g\), the following bounds hold.

There is a two-player static instance \(I_{0}\), such that
\label{claim:static-maintenance}
\[
 \mathbb E D_\Pi(T;I_{0})=\Omega(N_g(T))
 \qquad(T\to\infty).
\]

For every \(t_*\ge2\), there exists a dynamic instance \(I'\) with last population-event time \(t_*\) such that
\label{claim:dynamic-mismatch}
\label{cor:cumulative-mismatch-lower}
\begin{equation}
 \mathbb E D_\Pi(T;I')=\Omega\!\left(t_*+N_g(T)\right).
 \label{eq:cumulative-mismatch-lower}
\end{equation}
\end{theorem}

\paragraph{Proof idea.}
(1) For the static bound, choose a two-player market where one player cannot detect the other's departure without proposing to that player's arm. This proposal causes a mismatch when both players are present. The recovery condition therefore forces such proposals often enough even when no one leaves. Counting separate time intervals over which recovery is required gives the bound.
% For the static bound, consider two players \(p_1,p_2\) and two distinguished arms \(a_1,a_2\). Both players rank \(a_1\) first and \(a_2\) second. Arm \(a_1\) prefers \(p_1\) to \(p_2\), while every other arm prefers \(p_2\) to \(p_1\). When both players are present, the POSM is \(\{(p_1,a_1),(p_2,a_2)\}\); after \(p_1\) departs, the POSM assigns \(p_2\) to \(a_1\). Until \(p_2\) proposes to \(a_1\), its local feedback is identical in the coupled executions with and without the departure. Such a proposal necessarily causes mismatch in the static execution. The recovery condition therefore forces these proposals sufficiently often even when no player departs. Counting disjoint intervals over which recovery would be
% required yields the static \(\Omega_{\Pi,g}(N_g(T))\) lower bound.
(2) For the dynamic bound, we fix a population prefix that incurs expected mismatch proportional to \(t_*\) and leaves two players permanently present. We then compare this same instance with hypothetical departures of one player at later times. The recovery requirement forces further mismatches on the fixed instance. Combining these maintenance costs with the prefix cost yields the dynamic lower bound. The construction is independent of the evaluation horizon. The full proof appears in \Cref{sec:tradeoff-lower-proof}.

For every fixed recovery scale \(g\) covered by \Cref{thm:general-budget-upper}, the constructed protocol \(\Pi_g\) achieves worst-case static mismatch \(\Theta(N_g(T))\) as \(T\to\infty\). \Cref{thm:recovery-maintenance} gives a matching \(\Omega(N_g(T))\) lower bound for every fixed protocol satisfying \Cref{def:sublinear-mismatch}. 

Since the lower-bound constant may depend on the protocol, we next establish a uniform minimax characterization under a common recovery coefficient at \(\varepsilon=1/2\).

\begin{theorem}[Optimal static maintenance]
\label{thm:optimal-maintenance}
Fix \(K\ge2\) and a scale \(g\) satisfying the hypotheses of \Cref{thm:general-budget-upper}. For \(c>0\), let \(\mathcal C_{K,g}(c)\) be the class of legal protocols satisfying \Cref{def:sublinear-mismatch} and, for every legal finite-event instance \(I\) with last population-event time \(t_*\) and every \(h\ge c\,g(t_*)\), \(L_\Pi(h;I)\le h/2\).
There is a threshold \(c^{\star}_{K,g}=O_g(K^2)\) such that, for every fixed \(c\ge c^{\star}_{K,g}\),
\[
 \inf_{\Pi\in\mathcal C_{K,g}(c)}
 \ \sup_{I:\,t_*(I)=1}\mathbb E D_\Pi(T;I)
 =\Theta(N_g(T))
 \qquad(T\to\infty).
\]
\end{theorem}

The constructed protocol \(\Pi_g\) belongs to \(\mathcal C_{K,g}(c)\) for \(c\ge c^\star_{K,g}\) and attains this optimal asymptotic order. The proof is given in \Cref{sec:tradeoff-lower-proof}.

At the linear scale \(g(t)=t\), the dynamic lower bound in \Cref{thm:recovery-maintenance} matches the dependence on \(t_*\) and \(T\) achieved by SC-DA in \Cref{thm:known}, for fixed \(K\), \(t_*\ge2\), and \(T\ge t_*\).

\subsection{Representative Scales}
\label{sec:tradeoff-insights}

For the protocol classes in \Cref{thm:optimal-maintenance}, \(N_g(T)\) gives the optimal asymptotic order of worst-case static mismatch. \Cref{tab:representative-budgets} illustrates this count for representative recovery scales.

\begin{table}[ht]
\centering
\begin{tabular}{@{}ll@{}}
\toprule
Integer scale \(g(t)\), \(t\ge1\) & \(N_g(T)\), as \(T\to\infty\)\\
\midrule
\(t\) & \(\Theta(\log T)\)\\
\(\lceil t\log(e+t)\rceil\) & \(\Theta(\log T/\log\log T)\)\\
\(\lceil t\exp((\log t)^\delta)\rceil,\quad0<\delta<1\)
 & \(\Theta((\log T)^{1-\delta})\)\\
\(\lceil t^\alpha\rceil,\quad\alpha>1\) & \(\Theta(\log\log T)\)\\
\(\lceil t\exp((\log t)^\delta)\rceil,\quad\delta>1\)
 & \(\Theta(\log\log\log T)\)\\
\(2^t\) & \(\Theta(\log^*T)\)\\
\bottomrule
\end{tabular}
\caption{Representative iteration counts. Here \(\log^*T\) is the iterated logarithm.}
\label{tab:representative-budgets}
\label{cor:representative-budgets}
\end{table}
% The exponential row states only an iteration count; its computational
% applicability remains deferred to the author's discussion with the advisor.

% These orders follow from \(r_{j+1}=r_j+g(r_j)\). Writing \(y_j=\log r_j\) gives
% \begin{equation}
%  y_{j+1}-y_j=\log\!\left(1+\frac{g(r_j)}{r_j}\right).
%  \label{eq:budget-log-increment}
% \end{equation}

All shape parameters in the table are fixed rational numbers. The first five scales satisfy the hypotheses of \Cref{thm:general-budget-upper}, so \Cref{thm:optimal-maintenance} identifies their optimal static maintenance orders; their integer constructions and proofs appear in \Cref{sec:tradeoff-growth-proof}.

Beyond these representative scales, the iteration count satisfies the following asymptotic relations for nondecreasing integer scales \(g\) with \(g(t)=\Omega(t)\):

\begin{equation}
\begin{aligned}
 g(t)=t^{1+o(1)}
 &\quad\Longrightarrow\quad N_g(T)=\omega(\log\log T),\\
 g(t)=t^{\alpha+o(1)},\quad\alpha>1
 &\quad\Longrightarrow\quad N_g(T)=\Theta(\log\log T),\\
 g(t)=t^{\omega(1)}
 &\quad\Longrightarrow\quad N_g(T)=o(\log\log T).
\end{aligned}
\label{eq:budget-growth-regimes}
\end{equation}
The proofs of these relations and the table entries appear in \Cref{sec:tradeoff-growth-proof}.



% \begin{table}[ht]
% \centering
% \setlength{\tabcolsep}{5pt}
% \renewcommand{\arraystretch}{1.15}
% \begin{tabular}[t]{@{}ll@{}}
% \toprule
% Integer scale \(g(t)\) & \(N_g(T)\)\\
% \midrule
% \(t\)
%  & \(\Theta(\log T)\)\\
% \(\lceil t\log(e+t)\rceil\)
%  & \(\Theta(\log T/\log\log T)\)\\
% \(\lceil t\exp((\log t)^\delta)\rceil,\;0<\delta<1\)
%  & \(\Theta((\log T)^{1-\delta})\)\\
% \(\lceil t^\alpha\rceil,\;\alpha>1\)
%  & \(\Theta(\log\log T)\)\\
% \(\lceil t\exp((\log t)^\delta)\rceil,\;\delta>1\)
%  & \(\Theta(\log\log\log T)\)\\
% \(2^t\)
%  & \(\Theta(\log^*T)\)\\
% \bottomrule
% \end{tabular}
% \qquad
% \begin{tabular}[t]{@{}ll@{}}
% \toprule
% Growth of \(g(t)\) & \(N_g(T)\)\\
% \midrule
% \(\omega(t)\)
%  & \(o(\log T)\)\\
% \(t^{1+o(1)}\)
%  & \(\omega(\log\log T)\)\\
% \(t^{\alpha+o(1)},\;\alpha>1\)
%  & \(\Theta(\log\log T)\)\\
% \(t^{\omega(1)}\)
%  & \(o(\log\log T)\)\\
% \bottomrule
% \end{tabular}
% \caption{
% Representative scales (left) and general growth regimes (right),
% as \(T\to\infty\). Each condition in the right table implies the
% corresponding bound on \(N_g(T)\).
% All scales are nondecreasing and integer-valued, with \(g(t)\ge t\)
% for \(t\ge1\); the parameters \(\alpha,\delta\) are fixed.
% For \(r_0=2\) and \(r_{j+1}=r_j+g(r_j)\), writing \(y_j=\log r_j\)
% gives \(y_{j+1}-y_j=\log(1+g(r_j)/r_j)\).
% Here \(\log^*T\) is the iterated logarithm.
% Proofs appear in \Cref{sec:tradeoff-growth-proof}.
% }
% \label{tab:representative-budgets}
% \label{cor:representative-budgets}
% \label{eq:budget-log-increment}
% \label{eq:budget-growth-regimes}
% \end{table}
% % The exponential row states only an iteration count; its computational
% % applicability remains deferred to the author's discussion with the advisor.

==> sections/learning/arm-algorithm.tex <==
\begin{algorithm}[H]
\caption{SC-PC: arm service}
\label{alg:rcpc-arm}\hypertarget{scpc:arm}{}
\small
\algrenewcommand{\algorithmicindent}{0.75em}
\begin{algorithmic}[1]
\State At the first request, set \(a=e=\lambda=0\).
\Loop\Comment{Include all later empty rounds.}
  \State Observe the requester set \(R\).
  \ForAll{previously unseen handles \(i\in R\)}
    \State \(N_i\gets0;\quad U_i\gets0;\quad\operatorname{last}[i]\gets-\infty\)
  \EndFor
  \If{\(R\ne\varnothing\)}
    \If{\(\lambda>0\)}
      \State \(Q\gets C_a(R)\)
    \ElsIf{\(a\equiv0\pmod G\)}
      \State \(Q\gets R\)
    \Else
      \State \(Q\gets\{\min_{\prec}R\}\)
    \EndIf
    \State Choose \(i\in Q\) minimizing \(\operatorname{last}[i]\), breaking ties by \(\prec\).
    \State Accept \(i\), reject every other requester, and observe the private reward \(r\).
    \State \(N_i\gets N_i+1;\quad U_i\gets U_i+r\)
    \State \(\operatorname{last}[i]\gets a\)
  \EndIf
  \State \hypertarget{scpc:lease}{}\textbf{if} \(R=\varnothing\) \textbf{then} \(e\gets e+1\); \textbf{else} \(e\gets0\)
  \State \textbf{if} \(e\ge2\) \textbf{then} \(\lambda\gets\tau\); \textbf{else} \(\lambda\gets\max\{\lambda-1,0\}\)
  \State \(a\gets a+1\)
\EndLoop
\end{algorithmic}
\end{algorithm}

